Study, representation and applications of hypergraph minimal transversals

This work is part of the field of the hypergraph theory and focuses on hypergraph minimal transversal. The problem of extracting the minimal transversals from a hypergraph received the interest of many researchers as shown the number of algorithms proposed in the literature, and this is mainly due to the solutions offered by the minimal transversal in various application areas such as databases, artificial intelligence, e-commerce, semantic web, etc. In view of the wide range of fields of minimal transversal application and the interest they generate, the objective of this thesis is to explore new application paths of minimal transversal by proposing methods to optimize the extraction. This has led to three proposed contributions in this thesis. The first approach takes advantage of the emergence of Web 2.0 and, therefore, social networks using minimal transversal for the detection of important actors within these networks. The second part of research in this thesis has focused on reducing the number of hypergraph minimal transversal. A concise and accurate representation of minimal transversal was proposed and is based on the construction of an irredundant hypergraph, hence are calculated the irredundant minimal transversal of the initial hypergraph. An application of this representation to the dependency inference problem is presented to illustrate the usefulness of this approach. The last approach includes the hypergraph decomposition into partial hypergraph the local minimal transversal are calculated and their Cartesian product can generate all the hypergraph transversal sets. Different experimental studies have shown the value of these proposed approaches.

==> abbrev.tex <==
\chapter*{Liste des notations}\markboth{Liste des notations}{\textsc{Liste des notations}}
\begin{table}[!h]
\footnotesize{
\begin{tabular}{|r|r|}
\hline
$H^t$ & L'hypergraphe transversal � $H$ \\ \hline
$H'$ & L'hypergraphe irr�dondant associ� � $H$ \\ \hline
\textsc{tm} & Traverse minimale \\ \hline
$IM_H$ & Matrice d'incidence correspondant � l'hypergraphe $H$ \\ \hline
$\gamma_H$ & Ensemble des traverses de $H$ \\ \hline
$\mathcal{M}_H$ & Ensemble des traverses minimales de $H$ \\ \hline
$\tau$($H$) & Nombre de transversalit� de $H$ \\ \hline
$Supp\textsc{(}\textit{X}\textsc{)}$ & Support de l'ensemble des sommets $X$ \\ \hline
\textsc{tmm} & Traverse minimale multi-membre \\ \hline
$minsupp_u$ & Support minimal de "utilisateurs" d'un tri-concept\\ \hline
\textsc{Extent}($x$) & Extension du sommet $x$ \\ \hline
\textsc{df} & D�pendance fonctionnelle \\ \hline
$F^+$ & Fermeture d'un ensemble de \textsc{df}s \\ \hline
$D_r$ & Ensemble de toutes les \textsc{df}s satisfaites par une relation $r$ \\ \hline
\textsc{cover}($D_r$) & Couverture canonique de $D_r$  \\ \hline
Ag($t_i$, $t_j$) & Ensemble en accord des tuples $t_i$ et $t_j$ \\ \hline
\textsc{max}($D_r$, $A$) & Ensemble de tous les ensembles maximaux de $A$ dans une relation $r$ \\ \hline
c\textsc{max}($D_r$, $A$) & Compl�ment de \textsc{max}($D_r$, $A$) \\ \hline
\textsc{lhs}($D_r$, $A$) & Ensemble des pr�misses de $D_r$ pour un attribut $A$ \\ \hline
$Min$ & Minimalit� au sens de l'inclusion \\ \hline



\end{tabular}}
\end{table} 

==> chap4.tex <==
\chapter{Nouvelle représentation concise et exacte des traverses minimales par élimination de la redondance}\label{chap4}
\section{Introduction}
Dans le but d'optimiser l'extraction des traverses minimales, la réduction de l'espace de recherche se présente comme une solution potentielle évidente tant le nombre de traverses minimales d'un hypergraphe est généralement très important. Dans ce chapitre, nous proposons une représentation concise et exacte de l'ensemble des traverses minimales. Pour ce faire, nous introduisons la notion de traverse minimale irrédondante, basée sur trois nouveaux concepts que nous définissons, à partir desquels nous pouvons retrouver l'ensemble global de toutes les traverses minimales. Cette nouvelle approche, basée sur la notion de l'irrédondance dans les hypergraphes, a donné lieu à un algorithme d'extraction des traverses minimales, appelé \textsc{imt-extractor}. De plus, et afin de mettre en avant l'intérêt de cette nouvelle représentation des traverses minimales, nous proposons de l'appliquer au problème de l'inférence des dépendances fonctionnelles afin d'optimiser le calcul de la couverture minimale d'une relation donnée. Nous montrons que cette couverture minimale extraite à travers les traverses minimales irrédondantes est plus réduite que celle calculée par les approches existantes dans la littérature. 

\section{Motivations}\label{intro}

A la lumière du Chapitre \emph{2}, nous avons vu, dans la littérature, que plusieurs algorithmes ont été proposés pour l'extraction des traverses minimales d'un hypergraphe. A partir de cet état de l'art, nous mettons en exergue, dans cette section, les motivations qui nous ont conduit à la proposition d'une représentation concise des traverses minimales introduite dans le présent chapitre.

De tous les algorithmes qui se sont attachés à calculer les traverses minimales, aucun n'a fait, à ce jour, une complexité théorique polynomiale en la taille de l'entrée et de la sortie, comme l'a démontré Hagen \cite{thesehagen}. Ceci est dû essentiellement au fait que le nombre de traverses minimales peut être exponentiel par rapport à la taille de l'hypergraphe d'entrée.

Notre approche, inspirée des travaux de \cite{HamrouniSucc08}, est donc de chercher un sous-ensemble représentant de manière concise et exacte l'ensemble des traverses minimales. Ce sous-ensemble, qu'on appellera  ensemble irrédondant de traverses minimales, sera construit en considérant l'ensemble des hyperarêtes auxquelles appartient chaque sommet, appelé \emph{extension} et en construisant un hypergraphe irrédondant généralisé limité à un sous-ensemble des sommets initiaux ayant des extensions différentes que Kavvadias et Stavropoulos définissent comme des noeuds généralisés. L'espace de recherche s'en trouve alors réduit puisque plusieurs candidats ne seront pas générés par l'algorithme. Cette intuition se base sur le fait que si deux sommets $X$ et $Y$ appartiennent aux mêmes hyperarêtes, (\emph{i.e}, ils ont la même extension) et si $X$ appartient à une traverse minimale $T$, alors en substituant $X$ par $Y$ dans $T$ on obtient une nouvelle traverse minimale. En outre, le risque de redondance est éliminé puisque $Y$ n'est plus pris en compte dans l'exploration de l'espace de recherche.

Contrairement aux travaux de \cite{KavvadiasS05}, notre traitement s'effectue en prétraitement, et non en cours du processus de recherche des traverses minimales. Ainsi, à partir d'un sous-ensemble restreint de traverses minimales, notre approche permet de générer l'ensemble de toutes les traverses minimales. En ce sens, plus le nombre de sommets élagués est élevé, plus compact sera l'hypergraphe irrédondant et plus l'approche sera avantageuse. Ceci implique que notre approche cible un certain type d'hypergraphes qui, d'une part, renferment un très grand nombre de traverses minimales et, d'autre part, ont un nombre de transversalité élevé. De plus, ces hypergraphes sont composés par des larges ensembles de sommets appartenant aux mêmes hyperarêtes.

Dans la littérature, Medina et Nourine ont proposé une approche dont l'objectif est de réduire la taille de l'hypergraphe d'entrée \cite{Medina2005}. Les auteurs introduisent une nouvelle notion, appelé "les clones", dont le principe est le suivant : deux items (ou sommets) sont des clones si nous pouvons les permuter sans que ceci n'altère l'hypergraphe initial. Cette approche a pour principal objectif de réduire le nombre d'hyperarêtes de l'hypergraphe ($\mid \xi \mid$). En effet, si à partir d'un premier ensemble d'hyperarêtes, il est possible d'en déduire un second ensemble, l'ensemble $\xi$ s'en trouve considérablement réduit puisque le second ensemble serait éliminé. Cependant, notre approche propose de réduire la taille des hyperarêtes et non d'éliminer un ensemble d'hyperarêtes de l'hypergraphe d'entrée et c'est ce qui nous distingue des travaux de Medina et Nourine. Les deux notions ne sont pas équivalentes, comme le montre l'Exemple \ref{clone}.


\begin{example}\label{clone}
Soit un hypergraphe $H$ = (\{$1$, $2$, $3$, $4$, $5$, $6$\}, \{$e_1$ = \{$1$, $3$, $4$\}, $e_2$ = \{$1$, $3$, $5$\}, $e_3$ = \{$1$, $4$, $5$\}\}, $e_4$ = \{$3$, $4$, $5$\}, $e_5$ = \{$2$, $3$, $4$\}, $e_6$ = \{$2$, $4$, $5$\}\}). $H$ renferme $2$ sommets "clones", qui sont le $3$ et le $5$, mais aucun ensemble de sommets généralisés dans la mesure où chaque sommet de $H$ a une extension différente des autres sommets
\end{example}

\section{Notion d'irrédondance dans les hypergraphes}


L'approche que nous proposons pour calculer les traverses minimales d'un hypergraphe, consiste à réduire l'hypergraphe en le représentant de manière plus concise et sans perte d'information. Elle part de la constatation que deux ou plusieurs sommets qui ont la même extension, (\emph{i.e}, appartiennent exactement aux mêmes hyperarêtes) tiennent, à tour de rôle, la même position dans une traverse minimale mais ne peuvent y appartenir en même temps. 

Afin de remédier au problème du nombre extrêmement élevé des traverses minimales que peut contenir un hypergraphe, comme le montre l'exemple suivant, nous définissons la notion de l'irrdédondance dans les hypergraphes. L'ensemble des sommets est partitionné en des groupes de \emph{sommets généralisés} possédant un et un seul \emph{représentant}. Les sommets généralisés sont définis en se basant sur les hyperarêtes auxquelles appartient chaque sommet.
\begin{example}\label{expnb}
Soit $H = (\mathcal{X}, \xi)$ un hypergraphe tel que $\mathcal{X}$ = ($x_1$, $x_2$, \ldots, $x_{2n}$) et $\xi = (\{$$x_1$, $x_2$$\}$, $\{$$x_3$, $x_4$$\}$, \ldots, $\{$$x_{2n-1}$, $x_{2n}$$\}$). $H$ est de taille $2n$ mais renferme $2^n$ traverses minimales.
\end{example}
\`{A} partir de ces sommets généralisés, nous proposons de construire un hypergraphe généralisé (irrédondant) sur lequel seront calculées les traverses minimales irrédondantes qui serviront, par la suite, à déduire l'ensemble de toutes les traverses minimales d'un hypergraphe donné. Pour ce faire, nous proposons d'introduire à travers la Définition \ref{extension}, un nouveau concept, noté \emph{Extension}, qui nous permet de calculer pour chaque sommet l'ensemble exact des hyperarêtes auxquelles il appartient.

\begin{definition}\label{extension}
\textsc{Extension d'un sommet}\\
Soit $IM_H$ une matrice d'incidence correspondante à l'hypergraphe $H$ = ($\mathcal{X}$, $\xi$) et $x \in \mathcal{X}$. $E$ = $(e_1, e_2, \ldots, e_l)$ $\subseteq \xi $ est une extension de $x$ si  $x$ $\epsilon$ $e_i$, $\forall$ $e_i$ $\epsilon$ $E$. Nous noterons \textsc{Extent}($x$), l'extension de $x$ dans $IM_H$.
Le lien entre l'extension d'un sommet $x$ et son support est donné par la formule : $Supp\textsc{(}x\textsc{)}$ = $\mid$Extent($x$)$\mid$.
\end{definition}

\begin{example}
La Figure \ref{hyp2} illustre un hypergraphe  $H = (\mathcal{X}, \xi)$ tel que $\mathcal{X}$ = $\{$1, 2, 3, 4, 5, 6, 7, 8, 9$\}$ et  $\xi$ = $\{$$e_1$, $e_2$, $e_3$, $e_4$$\}$ avec $e_1$ = $\{$1, 2$\}$, $e_2$ = $\{$2, 3, 4$\}$, $e_3$ = $\{$3, 4, 5, 6, 7$\}$ et $e_4$ = $\{$7, 8, 9$\}$. Ainsi, la matrice d'incidence $IM_H$ correspondante à l'hypergraphe $H$ est décrite par le tableau \ref{contex}. Dans cet exemple, l'extension du sommet $2$ est égale aux hyperarêtes $e_1$ et $e_2$. Son support est, par conséquent, égal à $2$.
\end{example}


\begin{figure}
\begin{center}
\includegraphics[scale=0.7]{images/hgraphe14.eps}
\caption{Hypergraphe de 9 sommets et 4 hyperarêtes}\label{hyp2}
\end{center}
\end{figure}


\begin{table}
\begin{center}
\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|}
\hline
    {\bf } &   {\bf $\textbf{1}$} &   {\bf $\textbf{2}$} &   {\bf $\textbf{3}$} &   {\bf $\textbf{4}$} &   {\bf $\textbf{5}$} &   {\bf $\textbf{6}$} &   {\bf $\textbf{7}$} &   {\bf $\textbf{8}$}&   {\bf $\textbf{9}$}\\
\hline
  \textbf{$e_1$ = $\{1, 2\}$} &     $1$ &       $1$     &       0     &  0  &0 &0  & 0 &  0   & 0     \\
\hline
  \textbf{$e_2$ = $\{2, 3, 4\}$} &     0 &       $1$     &       $1$     &  $1$  &0 &0  & 0 &  0   & 0 \\
\hline
  \textbf{$e_3$ = $\{3, 4, 5, 6, 7\}$} &     0 &       0     &       $1$     &  $1$  &$1$ &$1$  & $1$ &  0   & 0  \\
\hline
  \textbf{$e_4$ = $\{7, 8, 9\}$} &     0 &       0     &       0     &  0  &0 &0  & $1$ &  $1$   & $1$    \\
  \hline
\end{tabular}
\caption{Matrice d'incidence correspondante à l'hypergraphe de la Figure\ref{hyp2}}\label{contex}
\end{center}
\end{table}




\section{Traverses Minimales irrédondantes : approche et algorithme}

Notre approche s'attache à réduire la taille de l'hypergraphe d'entrée dans le but d'obtenir une représentation concise et exacte, sans perte d'information, des traverses minimales. Cette dernière est basée sur deux notions importantes présentées par Kavvadias \emph{et al.} dans leurs travaux \cite{KavvadiasS05} : les sommets généralisés et l'hypergraphe généralisé.

\begin{definition}\label{classe}
\textsc{Sommets généralisés} \cite{KavvadiasS05}\\
Soit $H = (\mathcal{X}$, $\xi)$ un hypergraphe. L'ensemble $X$ $\subseteq$ $\mathcal{X}$ est un ensemble de sommets généralisés de $H$ si tous les sommets de $X$ appartiennent aux mêmes hyperarêtes de $\xi$.
\end{definition}

En d'autres termes et selon la Définition \ref{extension}, $X$ est considéré comme un ensemble de sommets généralisés où tous ses sommets ont la même extension. Ainsi, deux sommets $x_i$ et $x_j$ appartiennent à deux sommets généralisés différents si \textsc{Extent}($x_i$) $\neq$ \textsc{Extent}($x_j$).

Les ensembles de sommets généralisés, calculés à partir d'un hypergraphe $H$=($\mathcal{X}$, $\xi$) nous permettent de construire l'hypergraphe généralisé $H'$ associé à $H$. $H'$ est dit irrédondant puisque chaque sommet de $H'$ a une extension différente. Chaque ensemble de sommets généralisés a un et un seul \emph{représentant}, sélectionné selon la définition \ref{defrepre}.

\begin{definition}\label{defrepre}
\textsc{Représentant}\\
Soit $S$ un ensemble de sommets généralisés. $x_i$ est un \emph{Représentant} de $S$ si $x_i$ est le premier élément de $S$, $S$ étant trié par ordre lexicographique.
\end{definition}

\begin{example}\label{exp000}
Pour l'hypergraphe $H$ de la Figure \ref{hyp2}, constitué de 9 sommets, les extensions correspondantes à chacun des sommets sont indiquées dans le tableau \ref{extens}. Ces extensions nous permettent de déduire les représentants des sommets généralisés et la liste de leurs autres membres, décrits par le tableau \ref{classes}.
\begin{table}[htbp]
  \centering
\small{
\begin{tabular}{|r|r|}
\hline
    \textbf{Sommet} & \textbf{Extension} \\
\hline
  \bf{$1$} &     \{$e_1$\}  \\
\hline
  \bf{$2$} &     \{$e_1, e_2$\}   \\
\hline
  \bf{$3$} &     \{$e_2, e_3$\}    \\
\hline
  \bf{$4$} &     \{$e_2, e_3$\}     \\
  \hline
    \bf{$5$} &    \{$e_3$\}    \\
  \hline
  \bf{$6$} &     \{$e_3$\}  \\
  \hline
  \bf{$7$} &     \{$e_3, e_4$\} \\
  \hline
  \bf{$8$} &     \{$e_4$\} \\
  \hline
  \bf{$9$} &     \{$e_4$\} \\
  \hline
\end{tabular}
}
  \caption{Extensions des sommets de l'hypergraphe de la Figure \ref{hyp2}}\label{extens}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{|r|r|r|r|}
\hline
    \textbf{Sommets}  & \textbf{Représentants} & \textbf{Autres} \\
        \textbf{généralisés}  &  & \textbf{membres} \\
\hline
  $S_1$ = \{$1$\}   & \bf{$1$} &   -   \\
\hline
   $S_2$ = \{$2$\}   & \bf{$2$} &   -  \\
\hline
 $S_3$ = \{$3$, $4$\} & \bf{$3$} &   \bf{$4$}   \\
\hline
  $S_4$ =  \{$5$, $6$\}  & \bf{$5$} &  \bf{$6$}    \\
  \hline
 $S_5$ =  \{$7$\} &     \bf{$7$} & -   \\
  \hline
 $S_6$ =  \{$8$, $9$\}  & \bf{$8$} &   \bf{$9$}   \\
  \hline
\end{tabular}
\end{center}

\caption{Sommets généralisés}\label{classes}
\end{table}





\end{example}





\subsection{Cadre méthodologique}
%Dans le but de proposer une approche originale pour l'extraction des traverses minimales, nous avons usé des notions de la fouille de données
Notre représentation concise des traverses minimales repose sur deux notions importantes, expliquées dans la section 3 : les classes de substitution et surtout les \emph{Représentants}. Les classes de substitution, calculées à partir de l'hypergraphe $H$=($\mathcal{X}$, $\xi$) permettent tout d'abord de construire l'hypergraphe irrédondant $H'$ associé à $H$.

% Les traverses minimales irrédondantes vérifient des propriétés que nous proposons d'exposer dans cette section, avant d'introduire l'algorithme \textsc{smt-extractor}.


\begin{definition}\label{hypersucc} \textsc{Hypergraphe généralisé (irrédondant)}
Soit l'hypergraphe $H$=($\mathcal{X}$, $\xi$), $\mathcal{X'}$ $\subseteq$ $\mathcal{X}$ l'ensemble des représentants des différents sommets généralisés associés aux sommets de $H$ et $\xi'$ l'ensemble des hyperarêtes de $H$ privées des éléments de $\mathcal{X}$-$\mathcal{X'}$ et défini par $\xi' = \{e_i  \cap \mathcal{X'} , e_i  \cap \mathcal{X'} \ne \emptyset, \forall e_i \in \xi \}$. L'hypergraphe $H'$ = ($\mathcal{X'}$, $\xi'$) est appelé hypergraphe généralisé associé à $H$.

\end{definition}

Un hypergraphe généralisé $H'$ est un hypergraphe irrédondant puisqu'il n'existe pas deux sommets de $H'$ ayant la même extension.

\begin{example}\label{exppirr}
A la lecture du tableau \ref{classes}, nous aurons, pour l'hypergraphe de la figure \ref{hyp2}, $6$ ensembles de sommets généralisés, et les $6$ représentants correspondant : $1$,$ 2$, $3$, $5$, $7$, $8$. C'est uniquement à partir de ces derniers que sera construit l'hypergraphe irrédondant de la Figure \ref{hyp2_irr} dont les hyperarêtes sont $e'_1$ = $\{$1, 2$\}$, $e'_2$ = $\{$2, 3$\}$, $e'_3$ = $\{$3, 5, 7$\}$ et $e'_4$ = $\{$7, 8$\}$.
A partir de l'hypergraphe initial, nous remarquons que le sommet $7$, par exemple, est le seul à avoir une extension \{$3, 4$\}. $7$ sera donc le représentant d'une classe de substitution qui ne compte aucun autre élément. Par ailleurs, le sommet $4$ a la même extension que le sommet $3$, \emph{i.e}, \{$e_2, e_3$\}. Cette dernière n'est pas la même pour aucun autre sommet. Par conséquent, une classe de substitution est créée, dont le représentant est $3$ et qui renfermera les sommets $3$ et $4$.


\begin{figure}
\begin{center}
\includegraphics[scale=0.8]{images/hyp-irr.eps}
\caption{Hypergraphe irrédondant correspondant à l'hypergraphe de la Figure \ref{hyp2}}\label{hyp2_irr}
\end{center}
\end{figure}
\end{example}

\begin{definition} \textsc{Traverse minimale irrédondante}
Soit l'hypergraphe $H$=($\mathcal{X}$, $\xi$) et $H'$ = ($\mathcal{X'}$, $\xi'$) l'hypergraphe irrédondant associé à $H$, toute traverse minimale de $H'$ constitue une traverse minimale irrédondante de $H$.
\end{definition}

L'ensemble des traverses minimales de $H'$ (\emph{i.e.}, des traverses irrédondantes de $H$), $\mathcal{M}_{H'}$, permet de construire l'ensemble des traverses minimales de $H$.
En effet, toute traverse minimale irrédondante $T = \{x_1, ...x_l\}$ de $H$, composée de $l$ représentants $x_i$, $i = 1,..,l$ des classes de substitution $S_i, i = 1,..,l$ permet de générer $\prod_{i=1,l}|S_i|$ traverses minimales en remplaçant les représentants de chaque classe de substitution par les autres éléments de la classe.\\
Ainsi, dans l'exemple \ref{exp000}, la traverse minimale irrédondante $\{1,3,8\}$ formée des représentants des classes de substitution $S_1$, $S_3$ et $S_6$ de taille respective 1, 2 et 2 permet de construire 4 traverses minimales : $\{1,3,8\}$, $\{1,4,8\}$, $\{1,3,9\}$ et $\{1,4,9\}$.


\subsection{Etude de la complétude}
La construction de l'hypergraphe irrédondant $H'$ = ($\mathcal{X'}$, $\xi'$) à partir d'un hypergraphe initial $H$ =($\mathcal{X}$, $\xi$) repose sur trois propriétés importantes, présentées ci-dessous. Ces propriétés et leurs preuves montrent que toute traverse minimale de $H'$ est une traverse minimale de $H$ et que toute traverse minimale de $H$ peut être déduite à partir d'une traverse minimale de $H'$.

\begin{proposition}\label{prop1}
Toute hyperarête $e_i$, i $\in$ $\{1, 2, \ldots, m\}$, de $\xi$ est associée à exactement une hyperarête $e'_i$ of $\xi'$ définie par $e'_i$ = $e_i$ $\cap$ $\mathcal{X'}$ et inversement toute hyperarête $e'_i$, $i$ $\in$ $\{1, 2, \ldots, m\}$, de $\xi'$ correspond à une seule hyperarête $e_i$ de $\xi$.
\end{proposition}

\begin{proof}
Soit $e_i$ une hyperarête de $\xi$ et $e'_i$ $\in$ $\xi'$ tel que $e'_i$ = $e_i$ $\cap$ $\mathcal{X'}$.
Raisonnons par l'absurde et supposons que $e_i$ $\cap$ $\mathcal{X'}$ = $\emptyset$, alors $\exists$ $x$ $\in$ $e_i$ tel que $x$ $\not\in$ $\mathcal{X'}$ puisque $e_i$ $\neq$ $\emptyset$ selon la Définition \ref{hypergraphe} d'un hypergraphe.

Par ailleurs, la définition de $H'$, où $x$ $\not\in$ $\mathcal{X'}$, nous permet de déduire que $\exists$ $y$ $\in$ $\mathcal{X'}$ qui représente un ensemble de sommets généralisés de $x$ et, $x$ et $y$ ont la même extension.

Par conséquent, $y$ $\in$ $\mathcal{X'}$ et $y$ $\in$ $e_i$ contredisent le fait que $e_i$ $\cap$ $\mathcal{X'}$ = $\emptyset$. Ainsi, chaque hyperarête $e_i$ $\in$ $\xi$, $i$ $\in$ $\{1, 2, \ldots, m\}$ correspond à exactement une hyperarête $e'_i$ $\in$ $\xi'$, $\in$ $\{1, 2, \ldots, m\}$ définie par $e'_i$ = $e_i$ $\cap$ $\mathcal{X'}$.

Inversement à présent, soit $e'_i$ $\in$ $\xi'$ tel que $e'_i$ = $e_i$ $\cap$ $\mathcal{X'}$. Prouvons que $e'_i$ correspond à exactement une seule hyperarête $e_i$ de $\xi$.
Supposons qu'il existe une autre hyperarête $e_j$ de $\xi$, différente de $e_i$ telle que $e'_i$ = $e_j$ $\cap$ $\mathcal{X'}$. Donc, $\exists$ $y$ $\in$ $e_j$ tel que $y$ $\not\in$ $e_i$ puisque $e_i$ $\neq$ $e_j$ et \textsc{extent}($y$) $\neq$ \textsc{extent}($x$), $\forall x \in e_i$.
Ainsi, $y$ ou son représentant, $y'$, appartiennent à $\mathcal{X'}$ et $e_j$, et ils n'appartiennent pas à $e_i$. Ceci contredit le fait que $\mathcal{X'}$ $\cap$ $e_i$ = $\mathcal{X'}$ $\cap$ $e_j$.
En conclusion, toute hyperarête $e'_i$ de $\xi'$ correspond à exactement une seule hyperarête $e_i$ de $\xi$, $i$ $\in$ $\{1, 2, \ldots, m\}$.
\end{proof}


Nous présentons à présent diverses propriétés concernant la relation entre les traverses minimales irrédondantes et les traverses minimales.

\begin{proposition}
Toute traverse minimale $T$ de $H'$ est une traverse minimale de $H$, i.e., $\forall$ $T$ $\subseteq$ $\mathcal{X'}$, $T$ $\in$ $\mathcal{M}_{H'}$ $\Rightarrow$ $T$ $\in$ $\mathcal{M}_H$.
\end{proposition}

\begin{proof}
$T$ $\in$ $\mathcal{M}_{H'}$ $\Leftrightarrow$ $T$ $\cap$ $e'_i$ $\neq$ $\emptyset$, $\forall e'_i \in \xi'$.
Selon la Proposition \ref{prop1}, toute hyperarête $e'_i$ de $\xi'$ correspond à exactement une hyperarête $e_i$ of $\xi$. Soit $e_i \in \xi$ tel que $e'_i$ = $e_i \cap \mathcal{X'}$, $\forall$ i $\in$ $\{1, 2, \ldots, m\}$.
Nous avons $T$ $\cap$ $e'_i$ $\neq \emptyset$ $\forall$ i $\in$ $\{1, 2, \ldots, m\}$ $\Leftrightarrow$ $T$ $\cap$ $e_i \cap \mathcal{X'}$ $\neq \emptyset$.
Puisque $T$ $\subseteq$ $\mathcal{X'}$, ceci implique que $T$ $\cap$ $e_i$ $\neq \emptyset$ $\forall$ i $\in$ $\{1, 2, \ldots, m\}$. Ce qui prouve que $T$ $\in$ $\mathcal{M}_H$.
\end{proof}

\begin{proposition}(\textsc{complétude})
Toute traverse minimale $T$ de $H$ est associée à une traverse minimale $T'$ de $H'$.
\end{proposition}

\begin{proof}
Commençons par prouver que $T'$ est une traverse de $H'$.
Soit $T$ une traverse minimale de $H$ : $T$ = \{$x_{1}$, $x_{2}$, $\ldots$, $x_{k}$\} $\in \mathcal{M}_{H}$ avec $T$ $\cap e_i \neq \emptyset$, $\forall e_i \in \xi$. D'après les Définitions \ref{classe}, \ref{defrepre} et \ref{hypersucc}, nous avons $\forall x \in T$, $\exists x' \in \mathcal{X'}$ tel que \textsc{extent}($x$) = \textsc{extent}($x'$). De plus, puisque $T \in \mathcal{M}_{H}$, nous avons $\forall x_i \in T$ et $\forall x_j \in T$, $i$ $\neq$ $j$, \textsc{extent}($x_i$) $\neq$ \textsc{extent}($x_j$).\\

Si nous notons $T'$, le sous-ensemble de $\mathcal{X'}$ qui contient les représentants des éléments de $T$, nous avons $T'$ = \{$x'_{1}$, $x'_{2}$, $\ldots$ $x'_{l}$\} et $T'$ $\subset \mathcal{X'}$.
Puisque les éléments de $T$ et ceux de $T'$ ont la même extension et $T$ est une traverse de $H$, nous pouvons en déduire que $T'$ est une traverse de $H$. Nous avons alors : $T'$ $\cap$ $e_i$ $\neq \emptyset$, $\forall e_i \in \xi$. Or, comme $T'$ est un sous-ensemble de $\mathcal{X'}$, nous pouvons affirmer que :
$T' \cap \mathcal{X'} \cap e_i \neq \emptyset$, $\forall e_i \in \xi$\\
$\Leftrightarrow$ $T' \cap e'_i$ $\neq \emptyset$, $\forall e'_i \in \xi'$, suivant la Proposition 2. D'où, $T'$ est une traverse de $H'$.\\

Prouvons, à présent, que $T'$ est minimale dans $H'$. D'abord, nous pouvons noter que $T$ $\in$ $\mathcal{M}_{H}$ signifie que $\forall x \in T$, $\exists e_j \in \xi$ tel que $x \cap e_j \neq \emptyset$ et $T$ $\backslash$ \{$x$\} $\cap e_j$ = $\emptyset$ puisque $T$ est minimale, d'après l'hypothèse de départ.
Ensuite, puisque les éléments de $T$ et ceux de $T'$ ont la même extension, nous avons $\forall x' \in T'$, $\exists e_j \in \xi$ tel que $x' \cap e_j \neq \emptyset$ et $T'$ $\backslash$ \{$x'$\} $\cap e_j$ = $\emptyset$ \emph{(1)}.
Cependant, selon la définition de $H'$, $e'_j$ = $e_j$ $\cap \mathcal{X'}$ ce qui implique que $e'_j$ $\subseteq e_j$ \emph{(2)}.
\`{A} partir de \emph{(1)} et \emph{(2)}, nous pouvons déduire que la traverse $T'$ est minimale : $\forall x' \in T'$, $\exists e'_j \in \xi'$ tel que $T' \backslash\{x'\} \cap e'_j$=$\emptyset$.
\end{proof}

Dans ce qui suit, nous présentons le cadre méthodologique, basé sur cette approche, qui a donné naissance à l'algorithme \textsc{imt-extractor}, pour l'extraction des traverses minimales irrédondantes.


\subsection{Algorithme \textsc{imt-extractor}}
L'algorithme \textsc{imt-extractor}, dont le pseudo-code, est décrit par l'Algorithme \ref{algoglae2} prend en entrée une matrice d'incidence $IM_H$ (correspondante à l'hypergraphe d'entrée) et fournit en sortie l'ensemble des traverses minimales, noté $M_{H}$.


L'algorithme commence par calculer les extensions de chaque sommet de $\mathcal{X}$ à partir desquelles seront construits les différentes sommets généralisés (ligne 3). Cette tâche est effectuée par la procédure \textsc{Search-substitution}, dont le pseudo-code est décrit par l'Algorithme \ref{search}. Cette procédure fournit en sortie les différents sommets généralisés, conformément à la proposition \ref{classe}, avec pour chacun la liste des sommets qui le compose et son \emph{représentant}. A partir de ces données, une nouvelle matrice d'incidence $IM_{H'}$ associée à l'hypergraphe irrédondant $H'$ est générée à l'aide de la procédure \textsc{Change-hyp} selon la définition \ref{hypersucc}.

\begin{algorithm}[!h]
\LinesNumbered
\Entree{Une matrice d'incidence $IM_H$ associée à $H$ = ($\mathcal{X}$, $\xi$)}
 \Sortie{$\mathcal{M}_{H}$, l'ensemble des traverses minimales de $H$}
 \Deb{
 $M_{H'}$ = $\phi$;\\
   $Gen\_nodes$ := \textsc{Search-substitution}($IM_H$);\\
   $IM_{H'}$ = \textsc{Change-hyp}($IM_H$, $Gen\_nodes$);\\
   $\mathcal{M}_{H'}$ = \textsc{mmcs}($IM_{H'}$);\\
$\mathcal{M}_{H}$ = \textsc{get-all-mt}($\mathcal{M}_{H'}$, $Gen\_nodes$);\\
    \Retour{ $\mathcal{M}_{H}$ }
    }
    %$\mathcal{MT}$ = \textsc{get-all-mt}($MT_{irr}$, $Classes$);
     \caption{\textsc{imt-extractor}}
     \label{algoglae2}
\end{algorithm}

\textsc{imt-extractor} invoque un algorithme efficace d'extraction des traverses minimales, par exemple \textsc{mmcs} \cite{uno1} (line 5), présenté dans le chapitre $2$. Ce dernier calcule l'ensemble des traverses minimales de $H'$ selon une stratégie en profondeur d'abord et en utilisant une technique efficace pour tester la minimalité, basé sur la notion d'"hyperarêtes critiques" \cite{uno1}. \textsc{mmcs} retourne l'ensemble des traverses minimales de $H'$ qui représentent l'ensemble des traverses minimales irrédondantes de $H$. A noter que nous pouvons employer un autre algorithme que \textsc{mmcs} pour la réalisation de cette tâche. Notre choix a été conditionné par les performances supérieures à ses concurrents de l'algorithme \textsc{mmcs} de \cite{uno1}.



La procédure \textsc{Search-substitution($\mathcal{K}$)} calcule l'extension de chaque sommet $x$ à partir de la matrice d'incidence (ligne 5), \emph{i.e} l'ensemble des hyperarêtes auxquelles il appartient, à travers la fonction \textsc{Get-Extent}. Cette extension de $x$ est ensuite comparée aux extensions des différents \emph{représentants} des sommets généralisés existants (lignes 6-7). S'il existe déjà un représentant pour un ensemble de sommets généralisés $S$ qui a la même extension alors $x$ est ajouté à l'ensemble de sommets généralisés en question (ligne 8) et la variable booléenne $IsRep$ est mis à jour à \emph{False}, sinon (\emph{i.e}, $IsRep$ est égal à \emph{True}), un nouveau ensemble de sommets généralisés est créé pour le sommet $x$ qui en devient le représentant (ligne 11) et ce dernier est ajouté à la liste des \emph{Représentants} (ligne 12). Une fois, tous les sommets traités, la procédure renvoie à l'algorithme \textsc{imt-extractor} le représentant et la liste des sommets composant chaque ensemble de sommets généralisés calculé (ligne 13).
\begin{algorithm}[htbp]
{
\LinesNumbered
\Entree{Matrice d'incidence $IM_H$ associée à $H$}
%\KwIn {Context $\mathcal{K}$}
\Sortie{$Gen\_nodes$ : Ensemble de sommets généralisés
  }
\Deb
{
$Rep$ = $\emptyset$; /* Ensemble des Représentants*/ \\
\PourCh{$x \in \mathcal{X}$}
{

    $Extent$($x$) = \textsc{Get-Extent}($x$, $IM_H$);\\
    \PourCh{$y\in Rep$ }
    {
        IsRep = true ;\\
        \Si{$Extent$($x$) = $Extent$($y$)}
            {\textsc{Add-to-generalized-node}($Gen\_nodes$, $y$, $x$);\\
             IsRep = false ; }
    }
    \Si{IsRep = true}
    { \textsc{Add-Gen-node}($Gen\_nodes$, $x$, $Extent$($x$));\\
        $Rep$ = $Rep$ $\cup$ $x$;\\
    }
    }
\Retour($Gen\_nodes$);
}
}
  \caption{\textsc{Search-substitution}}
  \label{search}
\end{algorithm}


\begin{example}\label{lastexp}
Nous reprenons l'exemple \ref{exppirr} où on distingue $6$ sommets généralisés, dans l'hypergraphe initial $H$ de la Figure \ref{hyp2}, représentés par les sommets $1$, $2$, $3$, $5$, $7$ et $8$. Ces sommets calculés par la procédure \textsc{Search-substitution} permettent la construction de l'hypergraphe irrédondant $H'$ illustré par la Figure \ref{hyp2_irr}. La matrice d'incidence correspondante à $H'$ est ensuite utilisé par l'algorithme \textsc{mmcs} pour calculer toutes les traverses minimales $\mathcal{M}_{H'}$. \textsc{mmcs} donne ainsi en sortie l'ensemble $\{$$\{2,7\}$, $\{1,3,7\}$, $\{1,3,8\}$, $\{2,3,8\}$, $\{2,5,8\}$$\}$. Cet ensemble représente les traverses minimales irrédondantes de $H$. A partir de ces dernières, l'ensemble de toutes les traverses minimales de $H$ est, par la suite, généré comme le décrit la section suivante.
\end{example}


\subsection{Génération de toutes les traverses minimales}
Le processus de substitution pour la reconstruction de toutes les traverses minimales à partir de leur ensemble irrédondant est réalisé par la fonction \textsc{Get-all-Mt}, dont le pseudo-code est donné par l'Algorithme \ref{get-all-mt}.

\begin{algorithm}[htbp]
{
\LinesNumbered
\Entree{$\mathcal{M}_{H'}$, $Gen\_nodes$ }
%\KwIn {Context $\mathcal{K}$}
\Sortie{$\mathcal{M}_H$
  }
\Deb
{
$\mathcal{M}_H$ = $\emptyset$;\\
\PourCh{$T$ $\in$ $\mathcal{M}_{H'}$}{$\mathcal{M}_H$ = $\mathcal{M}_H$ $\cup$ $T$; \\\textsc{Substitute}($T$, $Gen\_nodes$, $\mathcal{M}_H$);}
\Retour($\mathcal{M}_H$);
}
}
  \caption{\textsc{Get-all-Mt}}
  \label{get-all-mt}
\end{algorithm}
\begin{algorithm}[htbp]
{
\LinesNumbered
\Entree{$T$, $Gen\_nodes$, $\mathcal{M}_H$ }
%\KwIn {Context $\mathcal{K}$}
\Deb
{
\PourCh{$x$ $\in$ $T$}{\PourCh{$G_n$ $\subset$ $Gen\_nodes$ tel que $x$ est un Représentant de $G_n$}{\Si{$\exists$ $y$ $\in$ $G_n$ et $x$ $\neq$ $y$}{$T$ = ($T$ $\backslash$ $x$) $\cup$ $y$;\\ $\mathcal{M}_H$ = $\mathcal{M}_H$ $\cup$ $T$;\\
\textsc{Substitute}($T$, $Gen\_nodes$, $\mathcal{M}_H$);}}}
}
}
  \caption{\textsc{Substitute}}
  \label{substi}
\end{algorithm}
 La fonction \textsc{Get-all-Mt} prend en entrée un ensemble de traverses minimales irrédondantes de $H$, i.e., l'ensemble des traverses minimales de $H'$. Dans chacunes de ces traverses irrédondantes, tout représentant est substitué successivement par tous les sommets qui appartiennent au même ensemble de sommets généralisés, par le biais de la fonction \textsc{Substitute}, presenté par l'Algorithme \ref{substi}. Pour revenir à notre exemple \ref{exppirr}, le tableau \ref{tmtotal} indique les traverses minimales de $H$ générées à partir de chaque traverse minimale irrédondante de $H'$ tout en méttant en évidence les sommets qui appartiennent au même ensemble de sommets généralisés. Au final, les \emph{15} traverses minimales de l'hypergraphe $H$ sont calculées à partir de seulement \emph{5} traverses minimales irrédondantes. Par exemple, les traverses minimales de $M_H$, $\{1,3,8\}$, $\{1,4,8\}$, $\{1,3,9\}$ et $\{1,4,9\}$, sont construites à partir de $\{1,3,8\}$ de $M_{H'}$ en remplaçant, respectivement, $3$ par $4$ et $8$ par $9$.


\begin{table}[!h]
\begin{center}
\begin{tabular}{|r|r|}
\hline
    \textsc{TMs irrédondantes} &   \textsc{TMs correspondantes} \\
\hline
  {\bf $\{2, 7\}$} &     {\bf $\{2, 7\}$}   \\
\hline
  {\bf $\{1, \textbf{3}, 7\}$} &     {\bf $\{1, \textbf{3}, 7\}$}, {\bf $\{1, \textbf{4}, 7\}$}  \\
\hline
  {\bf $\{1, \textbf{3}, \underline{8}\}$} &     {\bf $\{1, \textbf{3}, \underline{8}\}$}, {\bf $\{1, \textbf{4}, \underline{8}\}$}, {\bf $\{1, \textbf{3}, \underline{9}\}$}, {\bf $\{1, \textbf{4}, \underline{9}\}$}  \\
\hline
   {\bf $\{2, \textbf{3}, \underline{8}\}$} &     {\bf $\{2, \textbf{3}, \underline{8}\}$}, {\bf $\{2, \textbf{4}, \underline{8}\}$}, {\bf $\{2, \textbf{3}, \underline{9}\}$}, {\bf $\{2, \textbf{4}, \underline{9}\}$}   \\
  \hline
   {\bf $\{2, \textbf{5}, \underline{8}\}$} &     {\bf $\{2, \textbf{5}, \underline{8}\}$}, {\bf $\{2, \textbf{5}, \underline{9}\}$}, {\bf $\{2, \textbf{6}, \underline{8}\}$}, {\bf $\{2, \textbf{6}, \underline{9}\}$}  \\
  \hline
\end{tabular}
  \caption{Déduction de l'ensemble des traverses minimales}\label{tmtotal}
\end{center}
\end{table}





\begin{proposition}
Toute traverse minimale $T$ $\subseteq$ $\mathcal{X}$ générée par la fonction \textsc{Get-all-Mt} à partir de $T'$ appartenant à $\mathcal{M}_{H'}$, est une traverse minimale de $H$.
\end{proposition}

\begin{proof}
Soit $T'$ = \{$x'_{1}$, $x'_{2}$, $\ldots$ $x'_{k}$\} $\in$  $\mathcal{M}_{H'}$ et $T$ = \{$x_{1}$, $x_{2}$, $\ldots$ $x_{k}$\} générée par la fonction \textsc{Get-all-Mt} à partir de $T'$.
Commençons par prouver que $T$ est une traverse de $H$.

Par construction, $\forall x \in T$, $\exists$ $x'$ $\in$ $T'$ tel que \textsc{extent}($x$) = \textsc{extent}($x'$), ce qui implique que $x$ et $x'$ appartiennent exactement aux mêmes hyperarêtes de $H$.

De plus, $T'$ $\in$ $\mathcal{M}_{H'}$ $\Leftrightarrow$ $T'$ $\cap$ $e'_i$ $\neq$ $\emptyset$ $\forall e'_i \in \xi'$. Sachant que $e'_i$ = $e_i$ $\cap$ $\mathcal{X'}$ $\Rightarrow$ $e'_i$ $\subseteq$ $e_i$, nous avons alors $T'$ $\cap$ $e_i$ $\neq$ $\emptyset$ $\forall e_i \in \xi$ et puisque les éléments de $T$ et $T'$ ont la même extension, donc $T \cap e_i$ $\neq \emptyset$, $\forall e_i \in \xi$, et $T$ est ainsi une traverse de $H$.

Prouvons à présent que $T \in \mathcal{M}_H$.
Nous supposons que la traverse $T$ de $H$, générée à partir de $T'$, n'est pas minimale dans $H$. Dans ce cas, il existerait un sous-ensemble $T_0 \subset T$ qui est une traverse minimale de $H$. Soit $T_0$ cette traverse minimale : $T_0$ = \{$x_{1}$, $x_{2}$, $\ldots$ $x_{k-1}$\} $\subset T$ tel que $T_0 \cap e_i \neq \emptyset$, $\forall e_i \in \xi$.

$\forall x \in T_0$, $\exists x' \in T'$ tel que \textsc{extent}($x$) = \textsc{extent}($x'$).
Soit $T'_0$ le sous-ensemble de $T'$ contenant les représentants des éléments de $T_0$. $T'_0$ vérifie les propriétés suivantes :
\begin{description}
  \item[(1)] $T'_0 \cap e_i \neq \emptyset$, $\forall e_i \in \xi$;
  \item[(2)] $T'_0 \subset \mathcal{X'}$;
  \item[(3)] $T'_0 \subset T'$ et $T_0 \neq T'$;
\end{description}

A partir de (1) et (2), nous avons :\\
 $T'_0 \cap e_i \cap \mathcal{X'} \neq \emptyset$, $\forall e_i \in \xi$ $\Leftrightarrow T'_0 \cap e'_i \neq \emptyset$, $\forall$ $e'_i \in \xi'$.\\
Et par conséquent, $T'_0$ $\in \mathcal{M}_{H'}$.


D'après (3), $T'_0$, la traverse minimale de $H'$, est incluse et non égale à $T'$, ce qui constitue une contradiction avec le fait que nous avons supposé que $T'$ est une traverse minimale de $H'$. Ainsi, $T$ est minimale.

\end{proof}






\section{Etude expérimentale}
Afin d'évaluer l'intérêt de notre approche, nous avons étudié, à travers une série d'expérimentations, les performances de notre algorithme \textsc{imt-extractor}. Dans cet objectif, nous avons introduit la notion de taux de compacité qui est défini comme étant la proportion de traverses minimales qui peuvent être déduites à partir de l'ensemble des traverses minimales irrédondantes, sans perte d'information. De plus, nous comparons les temps d'exécution de notre algorithme \textsc{imt-extractor} à ceux de \textsc{ks} \cite{KavvadiasS05} et \textsc{mmcs} \cite{uno1}. Le temps global que requiert \textsc{imt-extractor} correspond à la somme de celui du prétraitement, du post-traitement et de l'extraction des traverses minimales irrédondantes réalisée par \textsc{mmcs} à partir de l'hypergraphe irrédondant. Notre algorithme est implémenté en \emph{C++} (compilé avec \emph{GCC} $4$.$1$.$2$) et nous avons utilisé une machine équipée d'un processeur Intel Core $i7$ CPU system, d'une capacité mémoire de $6$ Go RAM et du système d'exploitation Linux, \textsc{Ubuntu} $10$.$04$. L'algorithme \textsc{mmcs} utilisé au cours de ces expérimentations correspond à la version 3.1 disponible sur \emph{Hypergraph Dualization Repository} \cite{UnoSite}.

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|r||r|r|}
\hline
   &\emph{$p_l$} & \emph{$p_u $} &\emph{$|$$\mathcal{X}$$|$} & \emph{$|\xi|$} &  \emph{$|$Sommets\_Gen$|$}  & \emph{$\tau$(H)} \\
  \hline

    Accidents1 & 0.88 & 0.88 & 81   & 990  & 31  &  1  \\\hline
    Accidents2 & 0.90 & 0.90 & 336   & 10968  & 49   &  2    \\\hline
    Connect-Win & 0.05 & 0.11 & 79   & 12800 & 78  &  2  \\\hline

  \hline
  \end{tabular}
\end{center}
\caption{Caractéristiques des hypergraphes \emph{Accidents} et \emph{Connect}}\label{carac1}
\end{table}

Divers types d'hypergraphes ont été utilisés au cours de ces expérimentations. Le premier correspond à des hypergraphes générés à partir de la base de données "\textit{Accidents}", disponible depuis le \textsc{fimi} \emph{repository}\footnote[5]{Frequent Itemset Mining Datasets Repository, \emph{http://fimi.cs.helsinki.fi/data/}}, et depuis la base de données "\textit{Connect-4}" disponible à partir de l'\emph{\textsc{uci}} Machine Learning Repository \footnote[6]{UCI Machine Learning Repository, \emph{http://archive.ics.uci.edu/ml}}. Les caractéristiques de ces jeux de données sont résumés dans le tableau \ref{carac1}. La première et la seconde colonne, \emph{$p_l$} et \emph{$p_u $}, correspondent respectivement aux probabilités minimales et maximales pour qu'un sommet appartienne ou non à une hyperarête. En effet, un sommet appartient à une hyperarête avec une probabilité comprise entre $p_l$ et $p_u$  (0 $\leq$ $p_l$ $\leq$ $p_u$ $\leq$ 1). Une probabilité d'appartenance d'un sommet $x$ à une hyperarête $e$ est donnée par le quotient $\mid e \mid$/$\mid \mathcal{X} \mid$. La cinquième colonne indique le nombre de sommets généralisés générés pour chaque hypergraphe.

La dernière colonne correspond au nombre de transversalité $\tau$(H) de chaque hypergraphe, le nombre de transversalité étant la taille de la plus petite traverse minimale, i.e., le nombre de sommets la composant.




\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|}
\hline

   & \emph{$|$$\mathcal{M}_H$$|$} & \emph{$|$$\mathcal{M}_{H'}$$|$} &  $\theta$ \\
  \hline

    Accidents1  & 1961 & 1866 &  4,84\%\\\hline
    Accidents2   & 17486 & 17199 &  1,64\%\\\hline
    Connect-Win &  4587967 & 4423837 &  3,57\%\\\hline

  \end{tabular}
\end{center}
\caption{Statistiques sur les hypergraphes \emph{Accidents} et \emph{Connect}}\label{carac2}
\end{table}

La Table \ref{carac2} montre les statistiques relatives à l'hypergraphe initial et à l'hypergraphe irrédondant pour chaque jeu. La seconde colonne indique le nombre de traverses minimales que renferme l'hypergraphe d'entrée, $|$$\mathcal{M}_H$$|$. La troisième correspond au nombre de traverses minimales irrédondantes, $|$$\mathcal{M}_{H'}$$|$ tandis que la dernière colonne représente le taux de compacité $\theta$, calculé comme suit: ($|\mathcal{M}_H| - |\mathcal{M}_{H'}|) / |\mathcal{M}_H|$. Ce taux représente le pourcentage de traverses minimales qui peuvent être déduites à partir de l'ensemble des traverses minimales irrédondantes sans perte de l'information.



\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|}
\hline

   & Accidents1 & Accidents2&  Connect-Win \\
  \hline
   \textsc{mmcs}($H$)   & 0,301 & 2,787 &  88,491\\\hline
   \textsc{ks}($H$)   & 8,620 & - &  - \\\hline \hline
   \textsc{mmcs}($H'$)    & 0,001 & 2,366 &  84,015\\\hline
  \textsc{Get-all-Mt}($\mathcal{M}_{H'}$)   &  0,035 & 0,010 &  7,291\\\hline\hline
  \textsc{imt-extractor} ($H$)   &  0,036 & 2,376 & 91,306\\\hline

  \hline


  \end{tabular}
\end{center}
\caption{Temps de traitement sur les hypergraphes \emph{Accidents} et \emph{Connect} (en secondes)}\label{carac22}
\end{table}

En observant les statistiques récoltées sur les hypergraphes \emph{Accidents} et \emph{Connect-Win}, nous remarquons que le taux de compacité $\theta$ est très bas (variant entre 1.64\% et 4.84\%). Ceci peut être expliqué par le fait que les valeurs de $p_l$ et $p_u $, dans les différents hypergraphes, sont élevées mais principalement par les valeurs basses du nombre de transversalité, $\tau$, sur ces jeux de données. En effet, $\tau$ est égal à $1$ dans \emph{Accidents1} et à $2$ dans \emph{Accidents2} et \emph{ConnectWin}. A titre d'exemple, \emph{ConnectWin}, malgré des valeurs de $p_l$ et $p_u $ relativement basses, présente un taux de compacité égal à $4.48\%$, essentiellement dû à la valeur de $\tau$.


Dans le tableau \ref{carac22}, les temps d'exécution sont calculés en secondes et "-" signifie que le temps de traitement a dépassé les $3000$ secondes. Comme le met en évidence le tableau, l'algorithme \textsc{KS} est considérablement lent par rapport à \textsc{imt-extractor} et \textsc{mmcs}. Toutefois, le dernier algorithme nécessite approximativement le même temps pour extraire les traverses minimales à partir de $H$ et $H'$ pour \emph{Accidents2} et \emph{Connect-Win}. Cette constatation n'est pas valide pour \emph{Accidents1}. Par conséquent, pour ce dernier jeu de données, le temps d'exécution de \textsc{imt-extractor}, incluant pré-traitement et post-traitement, est moins important que celui requis par l'algorithme \textsc{mmcs}.

D'autre part, pour les jeux de données \emph{Accidents2} et \emph{Connect-Win}, l'hypergraphe irrédondant $H'$ et ses traverses minimales irrédondantes ne nous permettent pas d'optimiser sensiblement le temps de calcul des traverses minimales de $H$. Pour \emph{Connect-Win}, \textsc{mmcs} est même légèrement plus rapide que notre algorithme. Cette constatation est d'autant plus évidente lorsque les valeurs du taux de compacité de ces deux hypergraphes sont assez basses. En effet, le nombre de traverses minimales qui peuvent être déduites à partir de $\mathcal{M}_{H'}$ n'est pas assez important pour avoir un impact favorable sur notre approche. De la même manière, les trois hypergraphes testés ne renferment pas un très large ensemble de traverses minimales. Les expérimentations suivantes montreront que la réduction du temps d'exécution dépend fortement des valeurs de $|$$\mathcal{M}_H$$|$ et du nombre de transversalité $\tau$.
\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|r||r|r|}
\hline

   &\emph{$p_l$} & \emph{$p_u $} &\emph{$|$$\mathcal{X}$$|$} & \emph{$|\xi|$} & \emph{$|$Sommets\_Gen$|$} & \emph{$\tau$(H)} \\
  \hline

    $H1$ & 0.07 & 0.13 & 95   & 51  & 65   &  8   \\ \hline
    $H2$ & 0.06 & 0.11 & 99   & 101 & 64 &  9    \\ \hline
    $H3$ & 0.03 & 0.06 & 117   & 20005 & 68   &   4  \\ \hline\hline
    $H4$ & 0.05 & 0.05 & 60   & 20  & 20  &   20  \\ \hline

  \hline


  \end{tabular}
\end{center}
\caption{Caractéristiques des hypergraphes aléatoires}\label{carac3}
\end{table}


Dans le second volet de nos expérimentations, nous considérons un ensemble de trois hypergraphes ($H_1$, $H_2$ et $H_3$) générés de manière aléatoire. A partir d'un certain nombre de sommets $|\mathcal{X}|$, et d'un nombre d'hyperarêtes $|\xi|$, nous générons, de manière indépendante, $|\xi|$ ensembles de sommets tels que chacun d'eux correspond à une hyperarête, de l'hypergraphe, choisie de façon aléatoire. Le quatrième jeu de données ($H_4$) testé est un hypergraphe qui est composé de $|\mathcal{X}|$ sommets, $|\mathcal{X}| / 3$ hyperarêtes et la cardinalité de chaque hyperarête est égale à $3$. Ce dernier jeu de données est composé d'un ensemble réduit d'hyperarêtes mais d'un nombre de traverses minimales qui est exponentiel, i.e., égal à $3^{|\mathcal{X}| / 3}$.

Les caractéristiques de ces quatre hypergraphes aléatoires ($H1$, $H2$, $H3$ et $H4$) sont récapitulées dans le tableau \ref{carac3}.

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|}
\hline

   & \emph{$|$$\mathcal{M}_H$$|$} & \emph{$|$$\mathcal{M}_{H'}$$|$} &  $\theta$\\
  \hline

    $H1$ & 832564740 & 358392 &  99,95\%\\ \hline
    $H2$ & 265765380 & 189444 &  99,92\%\\ \hline
    $H3$ & 1693 & 1250 &  26,17\%\\ \hline\hline
    $H4$ &  $3^{20}$ & 1 &  99,99\% \\ \hline

  \hline


  \end{tabular}
\end{center}
\caption{Statistiques sur les hypergraphes aléatoires}\label{carac4}
\end{table}

Dans le but d'analyser plus en profondeur les traverses minimales irrédondantes utilisées par \textsc{imt-extractor} pour générer l'ensemble global des traverses minimales, considérons les statistiques données par le tableau \ref{carac4} sur les valeurs de \emph{$|$$\mathcal{M}_H$$|$}, \emph{$|$$\mathcal{M}_{H'}$$|$} et $\theta$. Nous remarquons que, pour $H1$ par exemple, \textsc{imt-extractor} se base sur seulement $358392$ traverses minimales irrédondantes pour retrouver les $832564740$ traverses minimales que renferme $H1$. Ce qui représente un taux de compacité de $99.95\%$. L'algorithme \textsc{mmcs} n'extrait donc que $0.05\%$ des traverses minimales qui sont utilisées, par la suite, par \textsc{imt-extractor}, pour retrouver l'ensemble \emph{$|$$\mathcal{M}_{H1}$$|$}. Les taux de compacité des trois autres hypergraphes traités varient entre $26.17\%$ et $99.99\%$ et dépendent beaucoup de la structure de ces hypergraphes, à savoir les valeurs de $p_l$ et $p_u$, mais aussi et surtout de leur nombre de transversalité. Généralement, plus ces valeurs sont basses, plus l'hypergraphe est éparse. Ceci implique, conformément à nos remarques préliminaires, un taux de compacité élevé et donc, un nombre très réduit de traverses minimales irrédondantes.


\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r||r|}
\hline

   & $H1$ & $H2$ & $H3$ & $H4$\\
  \hline
   \textsc{mmcs}($H$)   & 2083,79 & 766,19 &  124,69 & 245,61 \\\hline
   \textsc{ks}($H$)   & - & - &  1041,29 & 18,55 \\\hline \hline
   \textsc{mmcs}($H'$)    & 2,740 & 0,37 &  87,54 & 0,001\\\hline
  \textsc{Get-all-Mt}($\mathcal{M}_{H'}$)   &  11,69 & 1,53 &  0,03 & 19.80\\\hline\hline
  \textsc{imt-extractor} ($H$)   &  \textbf{14,43} & \textbf{1,90} &  \textbf{87,57} & \textbf{19.81}\\\hline

  \end{tabular}
\end{center}
\caption{Temps de traitement sur les hypergraphes aléatoires (en secondes)}\label{carac44}
\end{table}

Prenons à présent l'hypergraphe $H4$, notre approche représente les $3^{20}$ traverses minimales qu'il renferme par une et une seule traverse minimale irrédondante. Cette dernière est composée de tous les représentants des sommets généralisés de $H4$ dans la mesure où le nombre d'hyperarêtes est égal au nombre de transversalité \emph{$\tau$(H)}. Par ailleurs, nous remarquons que les valeurs de $p_l$ et $p_u$ sont les plus basses des hypergraphes du tableau \ref{carac4} et le nombre de transversalité est le plus élevé, i.e., égal à $20$

D'autre part, les valeurs de $\mathcal{M}_H$ et de $\mathcal{M}_{H'}$ nous permettent d'établir un lien entre le taux de compacité et le nombre de transversalité. Plus le nombre du transversalité est élevé, plus le taux de compacité l'est aussi. Nous remarquons de surcroît que la cardinalité de $\mathcal{M}_H$ pour ces quatre hypergraphes ($H1$, $H2$, $H3$ et $H4$) est largement plus élevée que les hypergraphes traités du tableau \ref{carac2}. Ainsi, nous pouvons affirmer que le taux de compacité est bien meilleur quand le nombre de traverses minimales est élevé. En effet, un très large ensemble de traverses minimales accroît la capacité d'\textsc{imt-extractor} à réduire la taille de l'hypergraphe d'entrée.

Le tableau \ref{carac44} récapitule les temps de traitement des algorithmes \textsc{mmcs}, \textsc{ks} et \textsc{imt-extractor}. Notre algorithme présente des performances intéressantes par rapport aux deux autres, en particulier sur l'hypergraphe $H_1$ où \textsc{mmcs} extrait les traverses minimales en $2084$ secondes alors que notre algorithme le fait en $14$ secondes. La différence est encore plus évidente sur $H_2$ où \textsc{mmcs} présente un temps de $766,19$ secondes alors que \textsc{imt-extractor} génère toutes les traverses en seulement $1,90$ seconde. \textsc{ks}, de son côté, ne s'exécute que sur les hypergraphes $H_3$ et $H_4$. Il est, d'ailleurs, le plus rapide des $3$ algorithmes considérés, sur ce dernier hypergraphe. Sur $H_1$ et $H_2$, il présente des temps de traitement supérieurs à $3000$ secondes. Ils ne sont donc pas pris en compte par le tableau \ref{carac44}. Notre représentation concise des traverses minimales permet donc d'optimiser singulièrement les temps de traitement sur ces hypergraphes aléatoires. De plus, les caractéristiques de ces hypergraphes nous permettent de dresser un profil du type d'hypergraphes sur lesquels \textsc{imt-extractor} est le plus efficace. En effet, notre algorithme se montre plus performant sur des hypergraphes ayant un nombre de transversalité élevé et tel que leurs hyperarêtes sont de petite taille et relativement disjoints. Au cours de nos expérimentations, nous avons pu remarquer que plus les hyperarêtes, d'un hypergraphe, sont disjoints, plus le nombre de sommets ayant une même extension est grand.

\section{Application de la représentation concise des traverses minimales au problème de l'inférence des dépendances fonctionnelles}
Nous avons introduit, dans les sections précédentes, une représentation concise et exacte des traverses minimales basée sur la notion de l'irrédondance de l'information. Pour mettre en exergue l'intérêt de notre approche, nous nous sommes intéressés au problème de l'inférence des dépendances fonctionnelles où les traverses minimales ont été utilisées comme une solution intéressante pour optimiser le calcul de la couverture minimale de toutes les dépendances fonctionnelles d'une relation $r$. Ainsi, nous montrons dans ce qui suit qu'il est possible de réduire la couverture minimale, qui permet de retrouver toutes les dépendances fonctionnelles satisfaites par une relation donnée. Nous introduisons ainsi le processus à suivre pour calculer cette couverture minimale et montrons comment retrouver l'ensemble de toutes les dépendances fonctionnelles.

\subsection{Notions de la théorie des BD relationnelles}

Avant de présenter l'application de notre représentation concise des traverses minimales, nous commençons par rappeler quelques définitions de la théorie des bases de données relationnelles ainsi que la problématique de l'inférence des dépendances fonctionnelles.

Dans le premier chapitre, nous avons exposé diverses problématiques où les traverses minimales peuvent présenter des solutions. Ceci est vrai pour le problème de l'inférence des dépendances fonctionnelles comme en témoignent les travaux recensés, dans la littérature, proposant d'optimiser le calcul du plus petit ensemble de dépendances fonctionnelles (appelé \emph{couverture minimale}) qui permet de retrouver l'ensemble de toutes les dépendances fonctionnelles satisfaites par une relation $r$, à travers l'application des traverses minimales.

Dans la suite, on note $R$ = \{$a_1$, $a_2$, \ldots, $a_n$\} un ensemble fini d'attributs, appelé aussi schéma de relation. Une relation $r$ est un ensemble fini de tuples \{$t_1$, $t_2$, \ldots, $t_n$\} de $R$. Soit un sous-ensemble d'attributs $X$, $u$[$X$] dénote la restriction du tuple $u$ de $r$ à $X$.

\begin{definition} \textsc{Dépendance fonctionnelle} \cite{Maier}\\
Soit un ensemble d'attributs $R$, une dépendance fonctionnelle (\textsc{df}) sur $R$ est une expression de la forme $X \rightarrow Y$, tel que $X$, $Y$ $\subseteq R$. Une \textsc{df} $X \rightarrow Y$ est satisfaite par $r$, noté $r \vDash X \rightarrow Y$, telle que $r$ est une relation sur $R$, si pour tout tuple $u$ et $v$ de $r$, nous avons $u[X]$ = $v[X]$ $\Rightarrow$ $u[Y]$ = $v[Y]$.

%Given a relation schema (set of attributes) $R$, a functional dependency (\textsc{fd}) overs $R$ is an expression $X \rightarrow Y$, where $X$, $Y$ $\subseteq R$. A \textsc{df} holds in $r$, denoted $r \vDash X \rightarrow Y$, such as $r$ is a relation over $R$, if all tuples $u$, $v$ $\in R$ with $u[X]$ = $v[X]$ satisfy also $u[Y]$ = $v[Y]$. Moreover, a functional dependency $X \rightarrow Y$ ($r \vDash X \rightarrow Y$) is minimal if and only if there is no proper subset $A$ of $X$ such as $r \vDash A \rightarrow Y$.
\end{definition}

Nous notons par $D_r$ l'ensemble de toutes les dépendances fonctionnelles satisfaites par la relation $r$.

\begin{definition}\textsc{Dépendance fonctionnelle minimale} \cite{Maier}
Une dépendance fonctionnelle $X \rightarrow Y$ satisfaite par $r$ ($r \vDash X \rightarrow Y$) est dite minimale si et seulement si $\not\exists Z \subset X$ tel que $r \vDash Z \rightarrow Y$.
\end{definition}



\begin{definition}\label{DefArms} \textsc{Axiomes d'Armstrong}
A partir d'un ensemble de dépendances fonctionnelles, nous pouvons en déduire d'autres grâce aux axiomes d'Armstrong qui représentent un système d'inférence complet et valide formé par les trois règles suivantes : \\
\begin{itemize}
  \item Réflexivité : Si $Y \subseteq X$, alors $X \rightarrow Y$.
  \item Augmentation : Si $X \rightarrow Y$, alors $XZ \rightarrow Y$ ; nous avons aussi $XZ \rightarrow YZ$.
  \item Pseudo-transitivité: Si $X \rightarrow Y$ et $YZ \rightarrow W$, alors $XZ \rightarrow W$.
\end{itemize}
\end{definition}



\begin{definition}\label{canon} \textsc{Fermeture d'un ensemble de \textsc{df}s} \cite{Maier}\\
Soient un ensemble $F$ de dépendances fonctionnelles. Nous appelons fermeture de $F$, notée $F^+$, les dépendances fonctionnelles contenant $F$ et tel qu'aucune autre dépendance fonctionnelle ne puisse être déduite de $F$.
\end{definition}

La fermeture d'un ensemble de dépendances fonctionnelles peut ainsi être considérée comme étant l'ensemble de toutes les \textsc{df}s pouvant être déduites par application des axiomes d'Armstrong. Cependant, cette fermeture dépend naturellement du schéma de relation $R$.

\begin{definition}\label{canon} \textsc{Couverture}\cite{Maier}\\
Soit $D$ et $G$ deux ensembles de dépendances fonctionnelles. $D$ est une couverture de $G$ si et seulement si $D^+$ = $G^+$.
\end{definition}

Autrement dit, si $r$ est une relation dans $R$ et $D$ un ensemble de dépendances fonctionnelles, si nous avons $r \vDash D$ alors toutes les \textsc{df}s de $D$ sont satisfaites par $r$. De plus, une dépendance $X \rightarrow Y$ est une \textit{conséquence} de $D$ si $r \vDash D$ implique $r \vDash X \rightarrow Y$ à travers les axiomes d'Armstrong, présentés dans la Définition \ref{DefArms}. De ce fait, si $D$ et $G$ sont deux ensembles de dépendances fonctionnelles, $D$ est considéré comme une couverture de $G$ si toutes les dépendances de $G$ sont des \emph{conséquences} de $D$.



\begin{definition}\label{canon} \textsc{Couverture canonique}\cite{Maier}\\
Soit $r$ une relation sur $R$ et $D_r$ l'ensemble de toutes les dépendances fonctionnelles satisfaites par $r$. La couverture canonique de $D_r$, noté \textsc{Cover}($D_r$) est définie comme suit :
\textsc{Cover}($D_r$) = \{$X \rightarrow Y \mid X \subset R$, $Y \in R$, $r \vDash X \rightarrow Y$ et $X \rightarrow Y$ est minimale\}.
\end{definition}


Notons, par ailleurs, que la couverture canonique est unique pour une relation $r$.

\begin{definition}\label{couvIrr} \textsc{Couverture irrédondante}\cite{Maier}\\
Une couverture $D$ est dite irrédondante si et seulement si $\not\exists$ $G \subset D$ tel que $G^+$ = $D^+$.
\end{definition}

\begin{definition}\label{couvMin} \textsc{Couverture minimale}\cite{Maier}\\
Une couverture est dite minimale si elle est canonique et irrédondante.
\end{definition}

L'ensemble $D_r$ peut avoir plusieurs couvertures équivalentes de différente tailles. Le problème d'inférence des dépendances fonctionnelles consiste donc à calculer la couverture de $D_r$ qui soit minimale selon la Définition \ref{couvMin}, et constituée du plus petit nombre de \textsc{df}s dont la fermeture permet de retrouver toutes les \textsc{df}s satisfaites par $r$.

\begin{example}\label{exphotel}
Considérons la relation $r$, synthétisée par le tableau \ref{rel}, où $A$, $B$, $C$, $D$ et $E$ représentent les attributs de $R$ \cite{ghada13}. Le tableau \ref{depr} résume l'ensemble de toutes les dépendances fonctionnelles satisfaites par $r$. Ainsi, nous pouvons remarquer que $AB \rightarrow D$ est une dépendance fonctionnelle satisfaite par $r$ mais qui n'est pas minimale puisque, pour $A \subseteq AB$, nous avons $r \vDash A \rightarrow D$. $AB \rightarrow D$ n'appartient donc pas à \textsc{Cover}($D_r$). $D_r$ est l'ensemble de toutes les dépendances fonctionnelles satisfaites par $r$.

\end{example}

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|r|r|}
\hline

   & $A$ & $B$ &  $C$ &  $D$ &  $E$ \\
  \hline

    $t_1$ & 1 & 100 &  1  & 2 & 50 \\
    $t_2$ & 4 & 101 &  1  & 2 & 50\\
    $t_3$ & 1 & 102 &  2  & 2 & 70\\
    $t_4$ & 1 & 200 &  1  & 2 & 50 \\
    $t_5$ & 2 & 101 &  3  & 3 & 100 \\
    $t_6$ & 2 & 200 &  1  & 3 & 70 \\
    $t_7$ & 1 & 100 &  3  & 2 & 50 \\ \hline
  \hline
  \end{tabular}
\end{center}
\caption{Une relation $r$}\label{rel}
\end{table}

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|}
\hline

 $BE \rightarrow A$ & $A \rightarrow D$ & $AB \rightarrow E$ \\
 $BD \rightarrow A$ & $CE \rightarrow D$ & $BD \rightarrow E$ \\
                    & $BE \rightarrow D$ & $AC \rightarrow E$ \\
                    &                   &  $CD \rightarrow E$ \\
 \hline
  \end{tabular}
\end{center}
\caption{L'ensemble \textsc{Cover}($D_r$) associé à la relation $r$}\label{depr}
\end{table}

Le problème de calcul d'une couverture minimale d'une relation $r$, plus connu sous le nom d'\emph{inférence de dépendances fonctionnelles}, a intéressé bon nombre de chercheurs. Cet intérêt est motivé, principalement, par les multiples applications de ce problème dans divers domaines, comme la conception et l'analyse des bases de données, l'optimisation des requêtes, etc. \cite{EiterIA}. Certains travaux se sont penchés sur la complexité du problème dans la mesure où l'espace de recherche des dépendances fonctionnelles est exponentiel en fonction du nombre d'attributs du schéma de relation considérée.

\subsection{Problème de l'inférence des dépendances fonctionnelles}
Heikki and R\"{a}ih\"{a} ont montré dans leurs travaux que le problème de l'inférence de dépendances fonctionnelles peut être réduit à un problème d'extraction des traverses minimales \cite{Mannila1994}. En effet, si $D_r$ représente toutes les dépendances fonctionnelles satisfaites par une relation $r$, la couverture minimale de $D_r$ est formée d'un ensemble de dépendances fonctionnelles dont les prémisses sont les traverses minimales d'un hypergraphe. Les hyperarêtes de ce dernier représentent les complémentaires des ensembles en accord de $r$, pour chaque attribut de $R$.

C'est en s'inspirant de cette idée que Lopes \emph{et al.} ont introduit l'algorithme \textsc{Dep-Miner} \cite{Lopes2000}, dont les expérimentations ont montré l'efficacité par rapport aux meilleurs algorithmes proposés dans la littérature et notamment celui de \cite{Huhtala98}.

Dans le but de mettre en évidence l'intérêt de notre représentation concise et exacte des traverses minimales pour le problème d'inférence des dépendances fonctionnelles, nous nous appuyons sur ce travail de Lopes \emph{et al.} qui introduisent les notions d'\emph{ensemble en accord} et d'\emph{ensemble maximal}.


\begin{definition}\label{agree} \textsc{Ensemble en accord}\cite{Lopes2000}\\
Soient $t_i$ et $t_j$ deux tuples et $X$ un ensemble d'attributs. Les tuples $t_i$ et $t_j$ sont \emph{en accord} sur $X$ si $t_i$[$X$] = $t_j$[$X$]. Ainsi, l'ensemble en accord de $t_i$ et $t_j$ est défini comme suit : Ag($t_i$, $t_j$) = \{$A \in R \mid t_i$[$A$] = $t_j$[$A$]\}. D'une manière générale, les ensembles en accord d'une relation $r$, que nous notons Ag($r$) sont calculés selon la formule suivante : \{Ag($t_i$, $t_j$) $\mid t_i$, $t_j \in r$, $t_i \neq t_j$\}.
\end{definition}

\begin{definition}\label{maxset} \textsc{Ensemble maximal}\\
Un ensemble maximal d'un attribut $A$ est un ensemble d'attributs $X \subseteq R$, maximal au sens de l'inclusion, et qui, à partir d'un ensemble de dépendances fonctionnelles $D$, ne détermine pas $A$.
L'ensemble de tous les ensembles maximaux de $A$ dans une relation $r$, noté \textsc{max}($D_r$, $A$), est défini comme suit :
\textsc{max}($D_r$, $A$) = \{$X \subseteq R \mid r \not\vDash X \rightarrow A$ et $\forall Y \subseteq R$, $X \subset Y$, $r \vDash Y \rightarrow A$\}. De plus, nous notons c\textsc{max}($D_r$, $A$) les compléments des ensembles maximaux \textsc{max}($D_r$, $A$) privés de $A$.
\end{definition}

\begin{lemma}
Soit $r$ une relation sur $R$, $A$ un attribut de $R$ et Ag($r$) tous les ensembles en accord de $r$. Nous avons \textsc{max}($D_r$, $A$) = Max\{ $X \in Ag(r) \mid A \not\in X$ \}.
\end{lemma}

L'ensemble de toutes les dépendances fonctionnelles $D_r$ peut être calculé à partir des ensembles maximaux. En effet, l'ensemble des prémisses (ou antécédents) de $D_r$ pour un attribut $A$, noté \textsc{lhs}($D_r$, $A$), est donné par la formule suivante : \textsc{lhs}($D_r$, $A$) = \{$X \subseteq R \mid r \vDash X \rightarrow A$ et $\forall X' \subset X$, $r \not\vDash X' \rightarrow A$\}. Par conséquent, l'ensemble des dépendances fonctionnelles de la forme $X \rightarrow A$ tel que $A \in R$ et $X \in$ \textsc{lhs}($D_r$, $A$) représente une couverture minimale de $D_r$.

Dans leur approche, Lopes \emph{et al.} ont remarqué que pour un attribut $A$, l'ensemble c\textsc{max}($D_r$, $A$) représente un hypergraphe simple dont les traverses minimales constituent les prémisses des dépendances fonctionnelles de telle sorte que : $\mathcal{M}_{c\textsc{max}(D_r, A)}$ = \textsc{lhs}($D_r$, $A$).

Pour une relation $r$, notre contribution intervient après la phase de calcul des différents c\textsc{max}, pour chaque attribut de $R$. A partir de chaque hypergraphe simple généré, nous extrayons les traverses minimales irrédondantes. En ce sens, les ensembles de sommets généralisés sont calculés et nous n'utiliserons que les attributs qui seront considérés comme des représentants. A partir de ces représentants, nous définissons une couverture minimale de $D_r$ qui est succincte, i.e., formée d'un ensemble de dépendances fonctionnelles plus réduit que celles calculées par les approches existantes. La couverture calculée par ces dernières peut être retrouvée, à partir de notre ensemble succinct, de deux manières différentes. La première consiste à substituer chaque représentant par un attribut appartenant au même ensemble de sommets généralisés. Ainsi, si $X \rightarrow A$ est une dépendance fonctionnelle satisfaite par $r$ et si $X$ est le représentant d'un ensemble $S$ de sommets généralisés tel que $S$ = \{$X$, $Z$\} alors nous avons  $r \vDash$ $Z \rightarrow$ $A$. Pour résumer donc, à partir des traverses minimales irrédondantes, nous générons les traverses minimales, comme démontré dans le chapitre $4$, et à partir de ces dernières nous retrouvons la couverture minimale telle que calculée par les approches existantes.

La seconde manière de retrouver cette couverture, est décrite par la proposition \ref{nj} et repose sur l'axiome de pseudo-transitivité d'Armstrong, présenté dans la Définition \ref{DefArms}.


\begin{proposition}\label{nj}
Soit $H$ un hypergraphe généré par c\textsc{max}($D_r$, $A$), $S$ un ensemble de sommets généralisés de $H$ et $X$ son représentant. $\forall$ $Y \in S$ et $Y \neq X$, nous avons : $r' \vDash$ $Y \rightarrow$ $X$ tel que $r' \subset r$ est une relation composée des tuples dont les ensembles en accord sont les éléments de \textsc{max}($D_r$, $A$).
\end{proposition}

\begin{proof}
Soit $A$ un attribut de $R$. L'hypergraphe associé à $A$ est $H_A$ = ($\mathcal{X}_A$, $\xi_A$) tel que $\mathcal{X}_A$ = $R$ $\cap$ $\xi_A$ et $\xi_A$ = c\textsc{max}($D_r$, $A$). L'ensemble c\textsc{max}($D_r$, $A$) représente les compléments des éléments de \textsc{max}($D_r$, $A$), lequel est constitué des éléments maximaux, au sens de l'inclusion, de Ag($r$) ne contenant pas l'attribut $A$.

De ce fait, $\forall T$ $\in$ \textsc{max}($D_r$, $A$) tel que $T$ $\subset$ $R$, nous avons $\forall X \in T$, $\exists$ deux tuples $t$ et $t'$ tel que $t$[$X$] = $t'$[$X$]. Puisque c\textsc{max}($D_r$, $A$) représente les compléments des éléments de \textsc{max}($D_r$, $A$) alors nous pouvons en déduire que $\forall T'$ $\in$ c\textsc{max}($D_r$, $A$) tel que $T'$ est le complément de $T$, alors $\forall X \in T'$, $t$[$X$] $\neq$ $t'$[$X$].

Considérons à présent un sommet généralisé $S$ de $H_A$ tel que $S$ = \{$X$, $Y$\} et $X$ est le représentant de $S$. \textsc{Extent}($X$) = \textsc{Extent}($Y$) $\Leftrightarrow$ $X$ et $Y$ appartiennent aux mêmes hyperarêtes de $H_A$ et donc aux mêmes éléments de c\textsc{max}($D_r$, $A$). Ainsi, $\forall T' \in$ c\textsc{max}($D_r$, $A$) tel que $X$ $\in$ $T'$ et $Y$ $\in$ $T'$, et $T'$ est le complément de $T$ tel que $T$ = Ag($t$, $t'$), alors : $t$[$X$] $\neq$ $t$[$Y$] et $t'$[$X$] $\neq$ $t'$[$Y$].

Donc, pour une relation composée des tuples $t$ et $t'$, nous avons les deux dépendances fonctionnelles conditionnelles de $r$, $Y \rightarrow$ $X$ et $X \rightarrow$ $Y$. Pour notre approche, nous n'aurons besoin que d'une seule. Celle où le représentant est l'antécédent (prémisse).
\end{proof}

En effet, pour un attribut donné, les éléments de l'ensemble \textsc{max} sont des ensembles en accord, maximaux au sens de l'inclusion. Ces éléments sont calculés à partir de couples de tuples. De ce fait, l'ensemble des tuples concernés représentent une relation $r'$ au sein de la relation initiale $r$. De plus, suivant la Définition \ref{agree}, les attributs appartenant à un même ensemble de sommets généralisés ont une même valeur au sein des tuples qui l'ont généré. Ainsi, la relation $r'$ satisfait naturellement les dépendances fonctionnelles de type $Y \rightarrow$ $X$ tel que $X$ est le représentant de l'ensemble des sommets généralisés auquel appartient $Y$.


\subsection{Etude de cas}
Dans l'objectif d'illustrer l'intérêt de notre représentation concise et exacte des traverses minimales pour le problème de l'inférence des dépendances fonctionnelles, nous présentons dans cette section une étude de cas qui détaille la manière dont nous calculons une couverture plus concise, que les approches existantes, de l'ensemble des dépendances fonctionnelles pour une relation donnée.

Reprenons ainsi la relation $r$ décrite par l'exemple \ref{exphotel}. Le tableau \ref{steps} montre les différentes étapes qui mènent à la couverture minimale \textsc{Cover}($D_r$) consistant en la génération des ensembles \textsc{lhs} pour chaque attribut de $r$. Le processus commence par calculer tous les ensembles en accord (ligne $1$), Ag($r$), selon la Définition \ref{agree}. Ensuite, et à partir de \textsc{Ag}($r$), les ensembles maximaux, pour chaque attributs, sont générés (ligne $3$). D'ailleurs, nous remarquons que les ensembles maximaux $B$ et $C$ sont, respectivement, $ACDE$ et $ABDE$. Ils n'ont pas été pris en considération dans la ligne $3$ car leurs compléments c\textsc{max}, privés de $B$ et $C$, sont égaux à l'ensemble vide. En ce sens, dans la ligne $4$, nous ne trouvons que les ensembles c\textsc{max} des attributs $A$, $D$ et $E$. Pour chaque attribut, chaque élément de c\textsc{max} représente une hyperarête de l'hypergraphe correspondant à l'attribut traité. Ainsi, si nous considérons par exemple l'attribut $A$, l'hypergraphe qui lui est associé ($H_1$) est constitué de deux hyperarêtes $e_1^1$ = $\{B\}$ et $e_1^2$ = $\{D, E\}$.

Au final, nous obtenons trois hypergraphes simples (ligne $5$). $H_1$ pour l'attribut $A$, $H_2$ pour $D$ et $H_3$ pour $E$. Un calcul des traverses minimales (ligne $6$) de chacun de ces hypergraphes permet de retrouver l'ensemble de dépendances fonctionnelles de \textsc{Cover}($D_r$). Pour $H_1$, l'ensemble des traverses minimales $\mathcal{M}_{H_1}$ renferme $BD$ et $BE$. Les deux dépendances fonctionnelles de \textsc{Cover}($D_r$) qui en découlent sont : $BD \rightarrow A$ et $BE \rightarrow A$. Selon le même principe, nous retrouvons les neuf autres \textsc{df} de \textsc{Cover}($D_r$) résumées par le Tableau \ref{depr}.

\begin{table}[htbp]
\begin{tabular}{|l|r|r|r|}
\hline
 & \multicolumn{3}{|c|}{Ag($r$) = \{$CDE$, $AD$, $D$, $ACDE$, $B$, $C$, $E$, $BC$,$ABDE$, $DE$, $ADE$\}}  \\
% & \multicolumn{3}{|c|}{$ABDE$, $DE$, $ADE$\}} \\
  \cline{2-4} \cline{2-4}
  & $A$ & $D$ & $E$ \\ \cline{2-4}
 & \textsc{max}($A$) =  & \textsc{max}($D$) = & \textsc{max}($E$) =  \\
 & \{$CDE$, $BC$\} & \{$E$, $BC$\} & \{$AD$, $BC$\} \\
  \cline{2-4}
\multirow{3}{*}{\rotatebox{90}{Lopes \emph{et al.}}} &   c\textsc{max}($A$) =  & c\textsc{max}($D$) =  & c\textsc{max}($E$) =  \\
& \{$B$, $DE$\} & \{$ABC$, $AE$\} & \{$BC$, $AD$\} \\
  \cline{2-4}
 &  $H_1 = (\mathcal{X}_1, \xi_1)$ & $H_2 = (\mathcal{X}_2, \xi_2)$  & $H_3 = (\mathcal{X}_3, \xi_3)$ \\
 & $\mathcal{X}_1$ = \{$B$, $D$, $E$\}  &    $\mathcal{X}_2$ = \{$A$, $B$, $C$, $E$\} &   $\mathcal{X}_1$ = \{$A$, $B$, $C$, $D$\} \\
 & $\xi_1$ = $\{$$e_1^1$ = $\{B\}$, & $\xi_2$ = $\{$$e_2^1$ = $\{A, B, C\}$, & $\xi_3$ = $\{$$e_3^1$ = $\{B, C\}$, \\
   & $e_1^2$ = $\{D, E\}$$\}$ &  $e_2^2$ = $\{A, E\}$$\}$  &  $e_3^2$ = $\{A, D\}$$\}$ \\ \cline{2-4}
&  $\mathcal{M}_{H_1}$ =  & $\mathcal{M}_{H_2}$ = \{$A$, & $\mathcal{M}_{H_3}$ = \{$AB$, $AC$,\\
& \{$BD$, $BE$\} & $BE$, $CE$\} &  $BD$, $CD$\} \\ \hline\hline
&  $S_1^1$ = $\{\textbf{B}\}$ & $S_1^2$ = $\{\textbf{A}\}$ & $S_1^3$ = $\{\textbf{B}, C\}$ \\\
&  $S_2^1$ = $\{\textbf{D}, E\}$ & $S_2^2$ = $\{\textbf{B}, C\}$ & $S_2^3$ = $\{\textbf{A}, D\}$ \\
\multirow{3}{*}{\rotatebox{90}{Notre contribution}}  &                  & $S_3^2$ = $\{\textbf{E}\}$ & \\ \cline{2-4}
  &  $H'_1 = (\mathcal{X'}_1, \xi'_1)$ & $H'_2 = (\mathcal{X'}_2, \xi'_2)$  & $H'_3 = (\mathcal{X'}_3, \xi'_3)$ \\
 &  $\mathcal{X'}_1$ = \{$B$, $D$\}  &    $\mathcal{X'}_2$ = \{$A$, $B$, $E$\} &   $\mathcal{X'}_1$ = \{$A$, $B$\} \\
 &  $\xi'_1$ = $\{$${e'}_1^1$ = $\{B\}$, & $\xi'_2$ = $\{$${e'}_2^1$ = $\{A, B\}$, & $\xi'_3$ = $\{$${e'}_3^1$ = $\{B\}$, \\
 &  ${e'}_1^2$ = $\{D\}$$\}$ &  ${e'}_2^2$ = $\{A, E\}$$\}$  &  ${e'}_3^2$ = $\{A\}$$\}$ \\ \cline{2-4}
&  $\mathcal{M}_{H'_1}$ = \{$BD$\} & $\mathcal{M}_{H'_2}$ = \{$A$, $BE$\} & $\mathcal{M}_{H'_3}$ = \{$AB$\}\\ \cline{2-4}
&  $BD \rightarrow A$ & $A \rightarrow D$; $BE \rightarrow D$ & $AB \rightarrow E$  \\ \hline
  \end{tabular}
\caption{Les étapes de génération de notre représentation concise de \textsc{Cover}($D_r$)}\label{steps}
\end{table}

Notre approche intervient juste après la construction des trois hypergraphes $H_1$, $H_2$ et $H_3$. Au lieu d'extraire les traverses minimales à partir de ces hypergraphes, nous en déduisons les hypergraphes irrédondants correspondants, $H'_1$, $H'_2$ et $H'_3$, à partir du calcul des ensembles de sommets généralisés (ligne $7$). Les représentants sont marqués en gras et les autres attributs sont supprimés des hypergraphes initiaux. Une fois les hypergraphes irrédondants construits (ligne $8$), nous calculons leurs traverses minimales correspondantes (ligne $9$) et qui nous permettront de représenter l'ensemble \textsc{Cover}($D_r$) de manière succincte.

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|}
\hline

 $BD \rightarrow A$ & $A \rightarrow D$ &  $BE \rightarrow D$ &$AB \rightarrow E$  \\
 \hline
  \end{tabular}
\end{center}
\caption{L'ensemble \textsc{Cover'}($D_r$)}\label{conciseDep}
\end{table}

Comme le montre le tableau \ref{conciseDep}, notre approche ne représente l'ensemble \textsc{Cover}($D_r$) qu'avec $4$ dépendances fonctionnelles absolues (satisfaites par $r$) alors que les approches existantes en calculent $9$. Cet ensemble est noté \textsc{Cover'}($D_r$). A partir de nos $4$ dépendances fonctionnelles, nous allons examiner la manière avec laquelle nous retrouvons l'ensemble \textsc{Cover}($D_r$) tel que représenté par le tableau \ref{depr} en suivant les deux méthodes présentées plus haut :

\begin{itemize}
  \item En appliquant le processus de substitution sur les dépendances fonctionnelles de l'ensemble \textsc{Cover'}($D_r$), nous retrouvons naturellement l'ensemble \textsc{Cover}($D_r$). Pour cela, nous avons besoin des ensembles de sommets généralisés déjà calculés. En effet, pour l'attribut $A$, $S_1^1$ ne contient que l'attribut $B$ alors que les attributs $D$ et $E$ appartiennent au même ensemble $S_2^1$ et puisque seulement le représentant $D$ a été considéré dans la construction de $H'_1$, nous n'avons généré qu'une dépendance fonctionnelle, pour $A$, qui est $BD \rightarrow A$. A partir donc de $S_2^1$, nous pouvons substituer $D$ par $E$ pour obtenir la dépendance fonctionnelle $BE \rightarrow A$. Cette dernière appartient effectivement dans \textsc{Cover}($D_r$). De même, pour l'attribut $D$, $CE \rightarrow D$ est obtenue à partir de $BE \rightarrow D$ puisque $B$ et $C$ appartiennent à $S_2^2$. Enfin, pour l'attribut $E$, trois dépendances fonctionnelles sont obtenues à partir de $AB \rightarrow E$ : $AC \rightarrow E$, $BD \rightarrow E$ et $CD \rightarrow E$.
  \item La seconde méthode qui permet de retrouver \textsc{Cover}($D_r$) à partir de \textsc{Cover'}($D_r$) serait d'appliquer l'axiome de pseudo-transitivité d'Armstrong. Selon la proposition \ref{nj}, deux attributs $X$ et $Y$ qui appartiennent au même ensemble de sommets généralisés, tel que $Y$ en est le représentant, sont liés par la dépendance fonctionnelle conditionnelle suivante : $X \rightarrow Y$. Cette relation serait "relative", et non absolue donc, car elle n'est vrai que par rapport à l'attribut à partir duquel les ensembles de sommets généralisés ont été calculés. Prenons l'exemple de l'attribut $A$ où nous avons généré deux ensembles $S_1^1$ et $S_2^1$. Ce dernier ensemble est composé des attributs $D$ et $E$. Nous pouvons donc déduire que la dépendance fonctionnelle $E \rightarrow D$ est satisfaite par les tuples qui ont permis de calculer les éléments de \textsc{max}($A$).

Analysons à présent l'ensemble \textsc{max}($A$), il est constitué de deux éléments $CDE$ et $BC$. Comme déjà expliqué, $CDE$ et $BC$ sont les ensembles en accord, de taille maximale, qui ne déterminent pas l'attribut $A$. L'ensemble en accord $CDE$ a été généré par les tuples $t_1$ et $t_2$ alors que $BC$ l'a été par les tuples $t_4$ et $t_6$. Si l'on considère donc uniquement la relation $r'$ formée par les tuples $t_1$, $t_2$, $t_4$ et $t_6$, nous pouvons aisément vérifier que la dépendance fonctionnelle $E \rightarrow D$ est satisfaite par $r'$. Puisque $r' \subset r$, $E \rightarrow D$ est dite alors dépendance fonctionnelle conditionnelle. Ainsi, en appliquant l'axiome de pseudo-transitivité d'Armstrong, nous avons : $E \rightarrow D$ et $BD \rightarrow A$ engendrent $BE \rightarrow A$. Nous retrouvons ainsi la troisième dépendance fonctionnelle de \textsc{Cover}($D_r$) ayant $A$ comme conclusion. Selon le même principe, nous générons pour l'attribut $D$, la dépendance fonctionnelle conditionnelle $C \rightarrow B$, et pour l'attribut $E$, $C \rightarrow B$ et $D \rightarrow A$. Le tableau \ref{dern} récapitule l'ensemble des \textsc{df}s conditionnelles qui, conjuguée à notre couverture succincte \textsc{Cover'}($D_r$) et à l'axiome d'Armstrong, permettent de retrouver \textsc{Cover}($D_r$).
\end{itemize}





\begin{table}[!h]
\begin{center}
\centering
\begin{tabular}{|l|r|r|r|}
\hline

 \multirow{2}{*}{\textsc{Cover'}($D_r$)} & $BD \rightarrow A$ & $A \rightarrow D$ &$AB \rightarrow E$  \\
 &  & $BE \rightarrow D$ & \\
 \hline
 \multirow{2}{*}{Dep. Fonct. Cond.} & $E \rightarrow D$ & $C \rightarrow B$ & $D \rightarrow A$ \\
 & &  $C \rightarrow B$ & \\ \hline
  \multicolumn{4}{c}{\textbf{+ Axiome d'Armstrong}} \\ \hline
\multirow{4}{*}{\textsc{Cover}($D_r$)} & $BE \rightarrow A$ & $A \rightarrow D$ & $AB \rightarrow E$ \\
  & $BD \rightarrow A$ & $CE \rightarrow D$ & $BD \rightarrow E$ \\
  &                  & $BE \rightarrow D$ & $AC \rightarrow E$ \\
  &                  &                   &  $CD \rightarrow E$ \\
 \hline
  \end{tabular}
\end{center}
\caption{Relation entre \textsc{Cover'}($D_r$) et \textsc{Cover}($D_r$)}\label{dern}
\end{table}



Ainsi, nous avons montré qu'en se basant sur notre représentation des traverses minimales, nous pouvons calculer une couverture minimale de l'ensemble de toutes les dépendances fonctionnelles d'une relation donnée encore plus réduite que ce que présentent les approches existantes. Ceci a pour objectif de réduire les temps de traitement nécessaires à la génération d'une couverture minimale et minimiser l'ensemble de dépendances fonctionnelles permettant de retrouver l'ensemble dans son intégralité d'une relation donnée. L'étude de cas illustre ainsi le processus proposé et donne un aperçu des dépendances fonctionnels "éliminées" dans la nouvelle couverture minimale que nous proposons.


\section{Conclusion}
Dans ce chapitre, nous avons introduit une nouvelle approche pour le calcul des traverses minimales d'un hypergraphe. Cette approche présente une représentation concise et exacte de l'ensemble des traverses minimales en se basant sur la notion d'irrédondance dans les hypergraphes. Ceci nous a permis d'introduire un cadre méthodologique qui a donné naissance à un nouvel algorithme \textsc{imt-extractor} pour l'extraction des traverses minimales. L'étude expérimentale a confirmé l'intérêt de notre approche sur un certain type d'hypergraphes présentant des taux de compacité intéressants. Néanmoins, au-delà de l'aspect expérimental, nous souhaitons prouver l'intérêt de cette nouvelle représentation des traverses minimales en montrant sa répercussion sur un des nombreux domaines d'application des traverses minimales. Pour cela, nous avons choisi d'appliquer notre représentation concise et exacte des traverses minimales au problème d'inférence des dépendances fonctionnelles, pour calculer la couverture minimale d'une relation donnée. Cette contribution a été publiée dans une conférence avec comité de lecture \cite{NidhalEGC2013}.Dans le chapitre suivant, nous introduisons une nouvelle méthode pour l'extraction des traverses minimales d'un hypergraphe en adoptant la stratégie "diviser pour régner". Nous démontrons que le partitionnement de l'hypergraphe initial en des hypergraphes partiels peut aussi s'avérer avantageux sur des hypergraphes particuliers.



==> chap4_bis.tex <==
\chapter{Application de la repr�sentation concise des traverses minimales au probl�me de l'inf�rence des d�pendances fonctionnelles}\label{chap4bis}
\section{Introduction}
Nous avons introduit dans le chapitre pr�c�dent une repr�sentation concise et exacte des traverses minimales bas�e sur la notion de l'irr�dondance de l'information. Pour mettre en exergue l'int�r�t de notre approche, nous nous sommes int�ress�s au probl�me de l'inf�rence des d�pendances fonctionnelles o� les traverses minimales ont �t� utilis�es comme une solution int�ressante pour optimiser le calcul de la couverture minimales de d�pendances fonctionnelles d'une relation $r$. Ainsi, nous montrons dans ce chapitre qu'il est possible de r�duire la couverture minimale, qui permet de retrouver toutes les d�pendances fonctionnelles satisfaites par une relation donn�e. Nous introduisons ainsi le processus � suivre pour calculer cette couverture minimale et montrons comment retrouver l'ensemble de toutes les d�pendances fonctionnelles.



\section{Notions de la th�orie des BD relationnelles}

Avant de pr�senter l'application de notre repr�sentation concise des traverses minimales, nous commen�ons par rappeler quelques d�finitions de la th�orie des bases de donn�es relationnelles ainsi que la probl�matique de l'inf�rence des d�pendances fonctionnelles.

Dans le premier chapitre, nous avons expos� diverses probl�matiques o� les traverses minimales peuvent pr�senter des solutions. Ceci est vrai pour le probl�me de l'inf�rence des d�pendances fonctionnelles comme en t�moignent les travaux recens�s, dans la litt�rature, proposant d'optimiser le calcul du plus petit ensemble de d�pendances fonctionnelles (appel� \emph{couverture minimale}) qui permet de retrouver l'ensemble de toutes les d�pendances fonctionnelles satisfaites par une relation $r$, � travers l'application des traverses minimales.

Dans la suite, on note $R$ = \{$a_1$, $a_2$, \ldots, $a_n$\} un ensemble fini d'attributs, appel� aussi sch�ma de relation. Une relation $r$ est un ensemble fini de tuples \{$t_1$, $t_2$, \ldots, $t_n$\} de $R$. Soit un sous-ensemble d'attributs $X$, u[$X$] d�note la restriction des tuples de $r$ � $X$.

\begin{definition} \textsc{D�pendance fonctionnelle} \cite{Maier}\\
Soit un ensemble d'attributs $R$, une d�pendance fonctionnelle (\textsc{df}) sur $R$ est une expression de la forme $X \rightarrow Y$, tel que $X$, $Y$ $\subseteq R$. Une \textsc{df} $X \rightarrow Y$ est satisfaite par $r$, not� $r \vDash X \rightarrow Y$, telle que $r$ est une relation sur $R$, si pour tout tuple $u$ et $v$ de $r$, nous avons $u[X]$ = $v[X]$ $\Rightarrow$ $u[Y]$ = $v[Y]$.

%Given a relation schema (set of attributes) $R$, a functional dependency (\textsc{fd}) overs $R$ is an expression $X \rightarrow Y$, where $X$, $Y$ $\subseteq R$. A \textsc{df} holds in $r$, denoted $r \vDash X \rightarrow Y$, such as $r$ is a relation over $R$, if all tuples $u$, $v$ $\in R$ with $u[X]$ = $v[X]$ satisfy also $u[Y]$ = $v[Y]$. Moreover, a functional dependency $X \rightarrow Y$ ($r \vDash X \rightarrow Y$) is minimal if and only if there is no proper subset $A$ of $X$ such as $r \vDash A \rightarrow Y$.
\end{definition}

Nous notons par $D_r$ l'ensemble de toutes les d�pendances fonctionnelles satisfaites par la relation $r$.

\begin{definition}\textsc{D�pendance fonctionnelle minimale} \cite{Maier}
Une d�pendance fonctionnelle $X \rightarrow Y$ satisfaite par $r$ ($r \vDash X \rightarrow Y$) est dite minimale si et seulement si $\not\exists Z \subset X$ tel que $r \vDash Z \rightarrow Y$.
\end{definition}



\begin{definition}\label{DefArms} \textsc{Axiomes d'Armstrong}
A partir d'un ensemble de d�pendances fonctionnelles, nous pouvons en d�duire d'autres gr�ce aux axiomes d'Armstrong qui repr�sentent un syst�me d'inf�rence complet et valide form� par les trois r�gles suivantes : \\
\begin{itemize}
  \item Reflexivit� : Si $Y \subseteq X$, alors $X \rightarrow Y$.
  \item Augmentation : Si $X \rightarrow Y$, alors $XZ \rightarrow Y$ ; nous avons aussi $XZ \rightarrow YZ$.
  \item Pseudo-transitivit�: Si $X \rightarrow Y$ et $YZ \rightarrow W$, alors $XZ \rightarrow W$.
\end{itemize}
\end{definition}



\begin{definition}\label{canon} \textsc{Fermeture d'un ensemble de \textsc{df}s} \cite{Maier}\\
Soient un ensemble $F$ de d�pendances fonctionnelles. Nous appelons fermeture de $F$, not�e $F^+$, le plus petit ensemble de toutes les d�pendances fonctionnelles contenant $F$ et tel qu'aucune autre d�pendance fonctionnelle, non pr�sente dans $F$, ne puisse �tre d�duite � travers les axiomes d'Armstrong.
\end{definition}

La fermeture d'un ensemble de d�pendances fonctionnelles peut ainsi �tre consid�r�e comme �tant l'ensemble de toutes les \textsc{df}s pouvant �tre d�duites par application des axiomes d'Armstrong. Cependant, cette fermeture d�pend naturellement du sch�ma de relation $R$.

\begin{definition}\label{canon} \textsc{Couverture}\cite{Maier}\\
Soit $D$ et $G$ deux ensembles de d�pendances fonctionnelles. $D$ est une couverture de $G$ si et seulement si $D^+$ = $G^+$.
\end{definition}

Autrement dit, si $r$ est une relation dans $R$ et $D$ un ensemble de d�pendances fonctionnelles, si nous avons $r \vDash D$ alors toutes les \textsc{df}s de $D$ sont satisfaites par $r$. De plus, une d�pendance $X \rightarrow Y$ est une \textit{cons�quence} de $D$ si $r \vDash D$ implique $r \vDash X \rightarrow Y$ � travers les axiomes d'Armstrong, pr�sent�s dans la D�finition \ref{DefArms}. De ce fait, si $D$ et $G$ sont deux ensembles de d�pendances fonctionnelles, $D$ est consid�r� comme une couverture de $G$ si toutes les d�pendances de $G$ sont des \emph{cons�quences} de $D$.



\begin{definition}\label{canon} \textsc{Couverture canonique}\cite{Maier}\\
Soit $r$ une relation sur $R$ et $D_r$ l'ensemble de toutes les d�pendances fonctionnelles satisfaites par $r$. La couverture canonique de $D_r$, not� \textsc{Cover}($D_r$) est d�finie comme suit :
\textsc{Cover}($D_r$) = \{$X \rightarrow Y \mid X \subset R$, $Y \in R$, $r \vDash X \rightarrow Y$ et $X \rightarrow Y$ est minimale\}.
\end{definition}


Notons, par ailleurs, que la couverture canonique est unique pour une relation $r$.

\begin{definition}\label{couvIrr} \textsc{Couverture irr�dondante}\cite{Maier}\\
Une couverture $D$ est dite irr�dondante si et seulement si $\not\exists$ $G \subset D$ tel que $G^+$ = $D^+$.
\end{definition}

\begin{definition}\label{couvMin} \textsc{Couverture minimale}\cite{Maier}\\
Une couverture est dite minimale si elle est canonique et irr�dondante.
\end{definition}

L'ensemble $D_r$ peut avoir plusieurs couvertures �quivalentes de diff�rente tailles. Le probl�me d'inf�rence des d�pendances fonctionnelles consiste donc � calculer la couverture de $D_r$ qui soit minimale selon la D�finition \ref{couvMin}, et constitu�e du plus petit nombre de \textsc{df}s dont la fermeture permet de retrouver toutes les \textsc{df}s satisfaites par $r$.

\begin{example}\label{exphotel}
Consid�rons la relation $r$, synth�tis�e par le tableau \ref{rel}, o� $A$, $B$, $C$, $D$ et $E$ repr�sentent les attributs de $R$. Le tableau \ref{depr} r�sume l'ensemble de toutes les d�pendances fonctionnelles satisfaites par $r$. Ainsi, nous pouvons remarquer que $AB \rightarrow D$ est une d�pendance fonctionnelle satisfaite par $r$ mais qui n'est pas minimale puisque, pour $A \subseteq AB$, nous avons $r \vDash A \rightarrow D$. $AB \rightarrow D$ n'appartient donc pas � \textsc{Cover}($D_r$). $D_r$ est l'ensemble de toutes les d�pendances fonctionnelles satisfaites par $r$.

\end{example}

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|r|r|}
\hline

   & $A$ & $B$ &  $C$ &  $D$ &  $E$ \\
  \hline

    $t_1$ & 1 & 100 &  1  & 2 & 50 \\
    $t_2$ & 4 & 101 &  1  & 2 & 50\\
    $t_3$ & 1 & 102 &  2  & 2 & 70\\
    $t_4$ & 1 & 200 &  1  & 2 & 50 \\
    $t_5$ & 2 & 101 &  3  & 3 & 100 \\
    $t_6$ & 2 & 200 &  1  & 3 & 70 \\
    $t_7$ & 1 & 100 &  3  & 2 & 50 \\ \hline
  \hline
  \end{tabular}
\end{center}
\caption{Une relation $r$}\label{rel}
\end{table}

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|}
\hline

 $BE \rightarrow A$ & $A \rightarrow D$ & $AB \rightarrow E$ \\
 $BD \rightarrow A$ & $CE \rightarrow D$ & $BD \rightarrow E$ \\
                    & $BE \rightarrow D$ & $AC \rightarrow E$ \\
                    &                   &  $CD \rightarrow E$ \\
 \hline
  \end{tabular}
\end{center}
\caption{L'ensemble \textsc{Cover}($D_r$) associ� � la relation $r$}\label{depr}
\end{table}

Le probl�me de calcul d'une couverture minimale d'une relation $r$, plus connu sous le nom d'\emph{inf�rence de d�pendances fonctionnelles}, a int�ress� bon nombre de chercheurs. Cet int�r�t est motiv�, principalement, par les multiples applications de ce probl�me dans divers domaines, comme la conception et l'analyse des bases de donn�es, l'optimisation des requ�tes, etc. \cite{EiterIA}. Certains travaux se sont pench�s sur la complexit� du probl�me dans la mesure o� l'espace de recherche des d�pendances fonctionnelles est exponentiel en fonction du nombre d'attributs du sch�ma de relation consid�r�e.

\section{Probl�me d'inf�rence des d�pendances fonctionnelles}
Heikki and R\"{a}ih\"{a} ont montr� dans leurs travaux que le probl�me de l'inf�rence de d�pendances fonctionnelles peut �tre r�duit � un probl�me d'extraction des traverses minimales \cite{Mannila1994}. En effet, si $D_r$ repr�sente toutes les d�pendances fonctionnelles satisfaites par une relation $r$, la couverture minimale de $D_r$ est form�e d'un ensemble de d�pendances fonctionnelles dont les pr�misses sont les traverses minimales d'un hypergraphe. Les hyperar�tes de ce dernier repr�sentent les compl�mentaires des ensembles en accord de $r$, pour chaque attribut de $R$.

C'est en s'inspirant de cette id�e que Lopes \emph{et al.} ont introduit l'algorithme \textsc{Dep-Miner} \cite{Lopes2000}, dont les exp�rimentations ont montr� l'efficacit� par rapport aux meilleurs algorithmes propos�s dans la litt�rature et notamment celui de \cite{Huhtala98}.

Dans le but de mettre en �vidence l'int�r�t de notre repr�sentation concise et exacte des traverses minimales pour le probl�me d'inf�rence des d�pendances fonctionnelles, nous nous appuyons sur ce travail de Lopes \emph{et al.} qui introduisent les notions d'\emph{ensemble en accord} et d'\emph{ensemble maximal}.


\begin{definition}\label{agree} \textsc{Ensemble en accord}\cite{Lopes2000}\\
Soient $t_i$ et $t_j$ deux tuples et $X$ un ensemble d'attributs. Les tuples $t_i$ et $t_j$ sont \emph{en accord} sur $X$ si $t_i$[$X$] = $t_j$[$X$]. Ainsi, l'ensemble en accord de $t_i$ et $t_j$ est d�fini comme suit : Ag($t_i$, $t_j$) = \{$A \in R \mid t_i$[$A$] = $t_j$[$A$]\}. D'une mani�re g�n�rale, les ensembles en accord d'une relation $r$, que nous notons Ag($r$) sont calcul�s selon la formule suivante : \{Ag($t_i$, $t_j$) $\mid t_i$, $t_j \in r$, $t_i \neq t_j$\}.
\end{definition}

\begin{definition}\label{maxset} \textsc{Ensemble maximal}\\
Un ensemble maximal d'un attribut $A$ est un ensemble d'attributs $X \subseteq R$, maximal au sens de l'inclusion, et qui, � partir d'un ensemble de d�pendances fonctionnelles $D$, ne d�termine pas $A$.
L'ensemble de tous les ensembles maximaux de $A$ dans une relation $r$, not� \textsc{max}($D_r$, $A$), est d�fini comme suit :
\textsc{max}($D_r$, $A$) = \{$X \subseteq R \mid r \not\vDash X \rightarrow A$ et $\forall Y \subseteq R$, $X \subset Y$, $r \vDash Y \rightarrow A$\}. De plus, nous notons c\textsc{max}($D_r$, $A$) les compl�ments des ensembles maximaux \textsc{max}($D_r$, $A$) priv�s de $A$.
\end{definition}

\begin{lemma}
Soit $r$ une relation sur $R$, $A$ un attribut de $R$ et Ag($r$) tous les ensembles en accord de $r$. Nous avons \textsc{max}($D_r$, $A$) = Max\{ $X \in Ag(r) \mid A \not\in X$ \}.
\end{lemma}

L'ensemble de toutes les d�pendances fonctionnelles $D_r$ peut �tre calcul� � partir des ensembles maximaux. En effet, l'ensemble des pr�misses (ou ant�c�dents) de $D_r$ pour un attribut $A$, not� \textsc{lhs}($D_r$, $A$), est donn� par la formule suivante : \textsc{lhs}($D_r$, $A$) = \{$X \subseteq R \mid r \vDash X \rightarrow A$ et $\forall X' \subset X$, $r \not\vDash X' \rightarrow A$\}. Par cons�quent, l'ensemble des d�pendances fonctionnelles de la forme $X \rightarrow A$ tel que $A \in R$ et $X \in$ \textsc{lhs}($D_r$, $A$) repr�sente une couverture minimale de $D_r$.

Dans leur approche, Lopes \emph{et al.} ont remarqu� que pour un attribut $A$, l'ensemble c\textsc{max}($D_r$, $A$) repr�sente un hypergraphe simple dont les traverses minimales constituent les pr�misses des d�pendances fonctionnelles de telle sorte que : $\mathcal{M}_{c\textsc{max}(D_r, A)}$ = \textsc{lhs}($D_r$, $A$).

Pour une relation $r$, notre contribution intervient apr�s la phase de calcul des diff�rents c\textsc{max}, pour chaque attribut de $R$. A partir de chaque hypergraphe simple g�n�r�, nous extrayons les traverses minimales irr�dondantes. En ce sens, les ensembles de sommets g�n�ralis�s sont calcul�s et nous n'utiliserons que les attributs qui seront consid�r�s comme des repr�sentants. A partir de ces repr�sentants, nous d�finissons une couverture minimale de $D_r$ qui est succincte, i.e., form�e d'un ensemble de d�pendances fonctionnelles plus r�duit que celles calcul�es par les approches existantes. La couverture calcul�e par ces derni�res peut �tre retrouv�e, � partir de notre ensemble succinct, de deux mani�res diff�rentes. La premi�re consiste � substituer chaque repr�sentant par un attribut appartenant au m�me ensemble de sommets g�n�ralis�s. Ainsi, si $X \rightarrow A$ est une d�pendance fonctionnelle satisfaite par $r$ et si $X$ est le repr�sentant d'un ensemble $S$ de sommets g�n�ralis�s tel que $S$ = \{$X$, $Z$\} alors nous avons  $r \vDash$ $Z \rightarrow$ $A$. Pour r�sumer donc, � partir des traverses minimales irr�dondantes, nous g�n�rons les traverses minimales, comme d�montr� dans le chapitre $4$, et � partir de ces derni�res nous retrouvons la couverture minimale telle que calcul�e par les approches existantes.

La seconde mani�re de retrouver cette couverture, est d�crite par la proposition \ref{nj} et repose sur l'axiome de pseudo-transitivit� d'Armstrong, pr�sent� dans la D�finition \ref{DefArms}.


\begin{proposition}\label{nj}
Soit $H$ un hypergraphe g�n�r� par c\textsc{max}($D_r$, $A$), $S$ un ensemble de sommets g�n�ralis�s de $H$ et $X$ son repr�sentant. $\forall$ $Y \in S$ et $Y \neq X$, nous avons : $r' \vDash$ $Y \rightarrow$ $X$ tel que $r' \subset r$ est une relation compos�e des tuples dont les ensembles en accord sont les �l�ments de \textsc{max}($D_r$, $A$).
\end{proposition}

\begin{proof}
Soit $A$ un attribut de $R$. L'hypergraphe associ� � $A$ est $H_A$ = ($\mathcal{X}_A$, $\xi_A$) tel que $\mathcal{X}_A$ = $R$ $\cap$ $\xi_A$ et $\xi_A$ = c\textsc{max}($D_r$, $A$). L'ensemble c\textsc{max}($D_r$, $A$) repr�sente les compl�ments des �l�ments de \textsc{max}($D_r$, $A$), lequel est constitu� des �l�ments maximaux, au sens de l'inclusion, de Ag($r$) ne contenant pas l'attribut $A$.

De ce fait, $\forall T$ $\in$ \textsc{max}($D_r$, $A$) tel que $T$ $\subset$ $R$, nous avons $\forall X \in T$, $\exists$ deux tuples $t$ et $t'$ tel que $t$[$X$] = $t'$[$X$]. Puisque c\textsc{max}($D_r$, $A$) repr�sente les compl�ments des �l�ments de \textsc{max}($D_r$, $A$) alors nous pouvons en d�duire que $\forall T'$ $\in$ c\textsc{max}($D_r$, $A$) tel que $T'$ est le compl�ment de $T$, alors $\forall X \in T'$, $t$[$X$] $\neq$ $t'$[$X$].

Consid�rons � pr�sent un sommet g�n�ralis� $S$ de $H_A$ tel que $S$ = \{$X$, $Y$\} et $X$ est le repr�sentant de $S$. \textsc{Extent}($X$) = \textsc{Extent}($Y$) $\Leftrightarrow$ $X$ et $Y$ appartiennent aux m�mes hyperar�tes de $H_A$ et donc aux m�mes �l�ments de c\textsc{max}($D_r$, $A$). Ainsi, $\forall T' \in$ c\textsc{max}($D_r$, $A$) tel que $X$ $\in$ $T'$ et $Y$ $\in$ $T'$, et $T'$ est le compl�ment de $T$ tel que $T$ = Ag($t$, $t'$), alors : $t$[$X$] $\neq$ $t$[$Y$] et $t'$[$X$] $\neq$ $t'$[$Y$].

Donc, pour une relation compos�e des tuples $t$ et $t'$, nous avons les deux d�pendances fonctionnelles conditionnelles de $r$, $Y \rightarrow$ $X$ et $X \rightarrow$ $Y$. Pour notre approche, nous n'aurons besoin que d'une seule. Celle o� le repr�sentant est l'ant�c�dent (pr�misse).
\end{proof}

En effet, pour un attribut donn�, les �l�ments de l'ensemble \textsc{max} sont des ensembles en accord, maximaux au sens de l'inclusion. Ces �l�ments sont calcul�s � partir de couples de tuples. De ce fait, l'ensemble des tuples concern�s repr�sentent une relation $r'$ au sein de la relation initiale $r$. De plus, suivant la D�finition \ref{agree}, les attributs appartenant � un m�me ensemble de sommets g�n�ralis�s ont une m�me valeur au sein des tuples qui l'ont g�n�r�. Ainsi, la relation $r'$ satisfait naturellement les d�pendances fonctionnelles de type $Y \rightarrow$ $X$ tel que $X$ est le repr�sentant de l'ensemble des sommets g�n�ralis�s auquel appartient $Y$.


\section{Etude de cas}
Dans l'objectif d'illustrer l'int�r�t de notre repr�sentation concise et exacte des traverses minimales pour le probl�me de l'inf�rence des d�pendances fonctionnelles, nous pr�sentons dans cette section une �tude de cas qui d�taille la mani�re dont nous calculons une couverture plus concise, que les approches existantes, de l'ensemble des d�pendances fonctionnelles pour une relation donn�e.

Reprenons ainsi la relation $r$ d�crite par l'exemple \ref{exphotel}. Le tableau \ref{steps} montre les diff�rentes �tapes qui m�nent � la couverture minimale \textsc{Cover}($D_r$) consistant en la g�n�ration des ensembles \textsc{lhs} pour chaque attribut de $r$. Le processus commence par calculer tous les ensembles en accord (ligne $1$), \textsc{Ag}($r$), selon la D�finition \ref{agree}. Ensuite, et � partir de \textsc{Ag}($r$), les ensembles maximaux, pour chaque attributs, sont g�n�r�s (ligne $3$). D'ailleurs, nous remarquons que les ensembles maximaux $B$ et $C$ sont, respectivement, $ACDE$ et $ABDE$. Ils n'ont pas �t� pris en consid�ration dans la ligne $3$ car leurs compl�ments c\textsc{max}, priv�s de $B$ et $C$, sont �gaux � l'ensemble vide. En ce sens, dans la ligne $4$, nous ne trouvons que les ensembles c\textsc{max} des attributs $A$, $D$ et $E$. Pour chaque attribut, chaque �l�ment de c\textsc{max} repr�sente une hyperar�te de l'hypergraphe correspondant � l'attribut trait�. Ainsi, si nous consid�rons par exemple l'attribut $A$, l'hypergraphe qui lui est associ� ($H_1$) est constitu� de deux hyperar�tes $e_1^1$ = $\{B\}$ et $e_1^2$ = $\{D, E\}$.

Au final, nous obtenons trois hypergraphes simples (ligne $5$). $H_1$ pour l'attribut $A$, $H_2$ pour $D$ et $H_3$ pour $E$. Un calcul des traverses minimales (ligne $6$) de chacun de ces hypergraphes permet de retrouver l'ensemble de d�pendances fonctionnelles de \textsc{Cover}($D_r$). Pour $H_1$, l'ensemble des traverses minimales $\mathcal{M}_{H_1}$ renferme $BD$ et $BE$. Les deux d�pendances fonctionnelles de \textsc{Cover}($D_r$) qui en d�coulent sont : $BD \rightarrow A$ et $BE \rightarrow A$. Selon le m�me principe, nous retrouvons les neuf autres \textsc{df} de \textsc{Cover}($D_r$) r�sum�es par le Tableau \ref{depr}.

\begin{table}[htbp]
\begin{tabular}{|l|r|r|r|}
\hline
 & \multicolumn{3}{|c|}{Ag($r$) = \{$CDE$, $AD$, $D$, $ACDE$, $B$, $C$, $E$, $BC$,$ABDE$, $DE$, $ADE$\}}  \\
% & \multicolumn{3}{|c|}{$ABDE$, $DE$, $ADE$\}} \\
  \cline{2-4} \cline{2-4}
  & $A$ & $D$ & $E$ \\ \cline{2-4}
 & \textsc{max}($A$) =  & \textsc{max}($D$) = & \textsc{max}($E$) =  \\
 & \{$CDE$, $BC$\} & \{$E$, $BC$\} & \{$AD$, $BC$\} \\
  \cline{2-4}
\multirow{3}{*}{\rotatebox{90}{Lopes \emph{et al.}}} &   c\textsc{max}($A$) =  & c\textsc{max}($D$) =  & c\textsc{max}($E$) =  \\
& \{$B$, $DE$\} & \{$ABC$, $AE$\} & \{$BC$, $AD$\} \\
  \cline{2-4}
 &  $H_1 = (\mathcal{X}_1, \xi_1)$ & $H_2 = (\mathcal{X}_2, \xi_2)$  & $H_3 = (\mathcal{X}_3, \xi_3)$ \\
 & $\mathcal{X}_1$ = \{$B$, $D$, $E$\}  &    $\mathcal{X}_2$ = \{$A$, $B$, $C$, $E$\} &   $\mathcal{X}_1$ = \{$A$, $B$, $C$, $D$\} \\
 & $\xi_1$ = $\{$$e_1^1$ = $\{B\}$, & $\xi_2$ = $\{$$e_2^1$ = $\{A, B, C\}$, & $\xi_3$ = $\{$$e_3^1$ = $\{B, C\}$, \\
   & $e_1^2$ = $\{D, E\}$$\}$ &  $e_2^2$ = $\{A, E\}$$\}$  &  $e_3^2$ = $\{A, D\}$$\}$ \\ \cline{2-4}
&  $\mathcal{M}_{H_1}$ =  & $\mathcal{M}_{H_2}$ = \{$A$, & $\mathcal{M}_{H_3}$ = \{$AB$, $AC$,\\
& \{$BD$, $BE$\} & $BE$, $CE$\} &  $BD$, $CD$\} \\ \hline\hline
&  $S_1^1$ = $\{\textbf{B}\}$ & $S_1^2$ = $\{\textbf{A}\}$ & $S_1^3$ = $\{\textbf{B}, C\}$ \\\
&  $S_2^1$ = $\{\textbf{D}, E\}$ & $S_2^2$ = $\{\textbf{B}, C\}$ & $S_2^3$ = $\{\textbf{A}, D\}$ \\
\multirow{3}{*}{\rotatebox{90}{Notre contribution}}  &                  & $S_3^2$ = $\{\textbf{E}\}$ & \\ \cline{2-4}
  &  $H'_1 = (\mathcal{X'}_1, \xi'_1)$ & $H'_2 = (\mathcal{X'}_2, \xi'_2)$  & $H'_3 = (\mathcal{X'}_3, \xi'_3)$ \\
 &  $\mathcal{X'}_1$ = \{$B$, $D$\}  &    $\mathcal{X'}_2$ = \{$A$, $B$, $E$\} &   $\mathcal{X'}_1$ = \{$A$, $B$\} \\
 &  $\xi'_1$ = $\{$${e'}_1^1$ = $\{B\}$, & $\xi'_2$ = $\{$${e'}_2^1$ = $\{A, B\}$, & $\xi'_3$ = $\{$${e'}_3^1$ = $\{B\}$, \\
 &  ${e'}_1^2$ = $\{D\}$$\}$ &  ${e'}_2^2$ = $\{A, E\}$$\}$  &  ${e'}_3^2$ = $\{A\}$$\}$ \\ \cline{2-4}
&  $\mathcal{M}_{H'_1}$ = \{$BD$\} & $\mathcal{M}_{H'_2}$ = \{$A$, $BE$\} & $\mathcal{M}_{H'_3}$ = \{$AB$\}\\ \cline{2-4}
&  $BD \rightarrow A$ & $A \rightarrow D$; $BE \rightarrow D$ & $AB \rightarrow E$  \\ \hline
  \end{tabular}
\caption{Les �tapes de g�n�ration de notre repr�sentation concise de \textsc{Cover}($D_r$)}\label{steps}
\end{table}

Notre approche intervient juste apr�s la construction des trois hypergraphes $H_1$, $H_2$ et $H_3$. Au lieu d'extraire les traverses minimales � partir de ces hypergraphes, nous en d�duisons les hypergraphes irr�dondants correspondants, $H'_1$, $H'_2$ et $H'_3$, � partir du calcul des ensembles de sommets g�n�ralis�s (ligne $7$). Les repr�sentants sont marqu�s en gras et les autres attributs sont supprim�s des hypergraphes initiaux. Une fois les hypergraphes irr�dondants construits (ligne $8$), nous calculons leurs traverses minimales correspondantes (ligne $9$) et qui nous permettront de repr�senter l'ensemble \textsc{Cover}($D_r$) de mani�re succincte.

\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|r|r|r|r|}
\hline

 $BD \rightarrow A$ & $A \rightarrow D$ &  $BE \rightarrow D$ &$AB \rightarrow E$  \\
 \hline
  \end{tabular}
\end{center}
\caption{L'ensemble \textsc{Cover'}($D_r$)}\label{conciseDep}
\end{table}

Comme le montre le tableau \ref{conciseDep}, notre approche ne repr�sente l'ensemble \textsc{Cover}($D_r$) qu'avec $4$ d�pendances fonctionnelles absolues (satisfaites par $r$) alors que les approches existantes en calculent $9$. Cet ensemble est not� \textsc{Cover'}($D_r$). A partir de nos $4$ d�pendances fonctionnelles, nous allons examiner la mani�re avec laquelle nous retrouvons l'ensemble \textsc{Cover}($D_r$) tel que repr�sent� par le tableau \ref{depr} en suivant les deux m�thodes pr�sent�es plus haut :

\begin{itemize}
  \item En appliquant le processus de substitution sur les d�pendances fonctionnelles de l'ensemble \textsc{Cover'}($D_r$), nous retrouvons naturellement l'ensemble \textsc{Cover}($D_r$). Pour cela, nous avons besoin des ensembles de sommets g�n�ralis�s d�j� calcul�s. En effet, pour l'attribut $A$, $S_1^1$ ne contient que l'attribut $B$ alors que les attributs $D$ et $E$ appartiennent au m�me ensemble $S_2^1$ et puisque seulement le repr�sentant $D$ a �t� consid�r� dans la construction de $H'_1$, nous n'avons g�n�r� qu'une d�pendance fonctionnelle, pour $A$, qui est $BD \rightarrow A$. A partir donc de $S_2^1$, nous pouvons substituer $D$ par $E$ pour obtenir la d�pendance fonctionnelle $BE \rightarrow A$. Cette derni�re appartient effectivement dans \textsc{Cover}($D_r$). De m�me, pour l'attribut $D$, $CE \rightarrow D$ est obtenue � partir de $BE \rightarrow D$ puisque $B$ et $C$ appartiennent � $S_2^2$. Enfin, pour l'attribut $E$, trois d�pendances fonctionnelles sont obtenues � partir de $AB \rightarrow E$ : $AC \rightarrow E$, $BD \rightarrow E$ et $CD \rightarrow E$.
  \item La seconde m�thode qui permet de retrouver \textsc{Cover}($D_r$) � partir de \textsc{Cover'}($D_r$) serait d'appliquer l'axiome de pseudo-transitivit� d'Armstrong. Selon la proposition \ref{nj}, deux attributs $X$ et $Y$ qui appartiennent au m�me ensemble de sommets g�n�ralis�s, tel que $Y$ en est le repr�sentant, sont li�s par la d�pendance fonctionnelle conditionnelle suivante : $X \rightarrow Y$. Cette relation serait "relative", et non absolue donc, car elle n'est vrai que par rapport � l'attribut � partir duquel les ensembles de sommets g�n�ralis�s ont �t� calcul�s. Prenons l'exemple de l'attribut $A$ o� nous avons g�n�r� deux ensembles $S_1^1$ et $S_2^1$. Ce dernier ensemble est compos� des attributs $D$ et $E$. Nous pouvons donc d�duire que la d�pendance fonctionnelle $E \rightarrow D$ est satisfaite par les tuples qui ont permis de calculer les �l�ments de \textsc{max}($A$).

Analysons � pr�sent l'ensemble \textsc{max}($A$), il est constitu� de deux �l�ments $CDE$ et $BC$. Comme d�j� expliqu�, $CDE$ et $BC$ sont les ensembles en accord, de taille maximale, qui ne d�terminent pas l'attribut $A$. L'ensemble en accord $CDE$ a �t� g�n�r� par les tuples $t_1$ et $t_2$ alors que $BC$ l'a �t� par les tuples $t_4$ et $t_6$. Si l'on consid�re donc uniquement la relation $r'$ form�e par les tuples $t_1$, $t_2$, $t_4$ et $t_6$, nous pouvons ais�ment v�rifier que la d�pendance fonctionnelle $E \rightarrow D$ est satisfaite par $r'$. Puisque $r' \subset r$, $E \rightarrow D$ est dite alors d�pendance fonctionnelle conditionnelle. Ainsi, en appliquant l'axiome de pseudo-transitivit� d'Armstrong, nous avons : $E \rightarrow D$ et $BD \rightarrow A$ engendrent $BE \rightarrow A$. Nous retrouvons ainsi la troisi�me d�pendance fonctionnelle de \textsc{Cover}($D_r$) ayant $A$ comme conclusion. Selon le m�me principe, nous g�n�rons pour l'attribut $D$, la d�pendance fonctionnelle conditionnelle $C \rightarrow B$, et pour l'attribut $E$, $C \rightarrow B$ et $D \rightarrow A$. Le tableau \ref{dern} r�capitule l'ensemble des \textsc{df}s conditionnelles qui, conjugu�e � notre couverture succincte \textsc{Cover'}($D_r$) et � l'axiome d'Armstrong, permettent de retrouver \textsc{Cover}($D_r$).
\end{itemize}





\begin{table}[htbp]
\begin{center}
\centering
\begin{tabular}{|l|r|r|r|}
\hline

 \multirow{2}{*}{\textsc{Cover'}($D_r$)} & $BD \rightarrow A$ & $A \rightarrow D$ &$AB \rightarrow E$  \\
 &  & $BE \rightarrow D$ & \\
 \hline
 \multirow{2}{*}{Dep. Fonct. Cond.} & $E \rightarrow D$ & $C \rightarrow B$ & $D \rightarrow A$ \\
 & &  $C \rightarrow B$ & \\ \hline
  \multicolumn{4}{c}{\textbf{+ Axiome d'Armstrong}} \\ \hline
\multirow{4}{*}{\textsc{Cover}($D_r$)} & $BE \rightarrow A$ & $A \rightarrow D$ & $AB \rightarrow E$ \\
  & $BD \rightarrow A$ & $CE \rightarrow D$ & $BD \rightarrow E$ \\
  &                  & $BE \rightarrow D$ & $AC \rightarrow E$ \\
  &                  &                   &  $CD \rightarrow E$ \\
 \hline
  \end{tabular}
\end{center}
\caption{Relation entre \textsc{Cover'}($D_r$) et \textsc{Cover}($D_r$)}\label{dern}
\end{table}



\section{Conclusion}
L'impact de notre repr�sentation concise et exacte de l'ensemble des traverses minimales est proportionnel � la diversit� des domaines d'application o� les traverses minimales peuvent pr�senter des solutions � bien des probl�matiques. Dans ce chapitre, nous avons appliqu� notre approche, pr�sent�e dans le chapitre $4$, au probl�me d'inf�rence des d�pendances fonctionnelles. Nous avons montr� qu'en se basant sur notre repr�sentation des traverses minimales, nous pouvons calculer une couverture minimale de l'ensemble de toutes les d�pendances fonctionnelles d'une relation donn�e encore plus r�duite que ce que pr�sentent les approches existantes. Ceci a pour double objectif de, et r�duire les temps de traitement n�cessaire � la g�n�ration d'une couverture minimale et minimiser l'ensemble de d�pendances fonctionnelles permettant de retrouver l'ensemble dans son int�gralit� d'une relation. L'�tude de cas, pr�sent�e � la fin de ce chapitre illustre le processus propos� et donne un aper�u des d�pendances fonctionnels "�limin�es" dans la nouvelle couverture minimale que nous proposons. Dans le chapitre suivant, nous introduisons une nouvelle m�thode pour l'extraction des traverses minimales d'un hypergraphe en adoptant la strat�gie "diviser pour r�gner". Nous d�montrons que le partitionnement de l'hypergraphe initial en des hypergraphes partiels peut aussi s'av�rer avantageux sur des hypergraphes particuliers.

